Semantic Attention Flow Fields for Monocular Dynamic Scene Decomposition

From video, we reconstruct a neural volume that captures time-varying color, density, scene flow, semantics, and attention information. The semantics and attention let us identify salient foreground objects separately from the background across spacetime. To mitigate low resolution semantic and attention features, we compute pyramids that trade detail with whole-image context. After optimization, we perform a saliency-aware clustering to decompose the scene. To evaluate real-world scenes, we annotate object masks in the NVIDIA Dynamic Scene and DyCheck datasets. We demonstrate that this method can decompose dynamic scenes in an unsupervised way with competitive performance to a supervised method, and that it improves foreground/background segmentation over recent static/dynamic split methods. Project Webpage: https://visual.cs.brown.edu/saff

==> alg/alg_clustering.tex <==
\begin{algorithm}[t]
    \caption{\textbf{Saliency-aware Clustering.} The input is $N$ semantic feature images rendered for each of the training spacetime viewpoint ($N \times H \times W \times D$). $H$, $W$ are image height and width, and $D$ is the semantics feature dimension. }
    \label{alg:cluster}
    \begin{algorithmic}
        \Require  $inputs \in R^{N \times H \times W \times D}, saliency \in R^{N \times H \times W \times 1}$
        \State $interval \gets 5$, $k_{max} \gets 25$, $elbow \gets 0.975$
        \State $percentage \gets 70$, $th_{merge} \gets 0.5$, $th_{sal} \gets 0.07$
        \State $seed \gets 1234$, $n_{iter} \gets 300$, $n_{redo} \gets 10$
        %\Require $n \geq 0$
        \Ensure $C \in R^{K \times D}$, $M = \{...\}$, $S = [...]$ 
        %\State $y \gets 1$
        %\State $X \gets x$
        %\State $N \gets n$
        \State  $N, H, W, D \gets inputs$.shape
        \State $feat \gets inputs$ reshaped to $((N \times H \times W), D)$
        \State $sampled \gets feat[::interval, :]$
        \State $k \gets 1$
        \State $dists \gets [ ]$
        \While{$k \neq k_{max}$}
        \State $clu \gets Kmeans(D, k, n_{iter}, n_{redo}, seed)$
        \State $clu$.train($sampled$)
        \State $labels \gets clu$($feat$)
        \State $dist \gets$ squared distances of points to centroids of $clu$ 
        \State $dists$.append($dist$)
        \If{$k \geq 2$ and $dists[-1] > elbow \times dists[-2]$}
        \State break
        %    \State $X \gets X \times X$
        %    \State $N \gets \frac{N}{2}$  \Comment{This is a comment}
        %\ElsIf{$N$ is odd}
        %    \State $y \gets y \times X$
        %    \State $N \gets N - 1$
        \EndIf
        \State $k \gets k+1$
        \EndWhile
        \State $C \gets clu$.centroids, $K \gets C$.shape$[0]$
        \State $Sim \gets \{\}$
        \State $c_1 \gets 0$  
        \While{$c_1 < K$}
        \State $c_2 \gets 0$
        \While{$c_2 < K$}
        \State $Sim[c_1, c_2]$ $\gets$ ($C[c_1]\cdot C[c_2]$) / ($||C[c_1]||$ $\times$ $||C[c_2]||$)
        \State $c_2 \gets c_2 + 1$  
        \EndWhile
        \State $c_1 \gets c_1 + 1$  
        \EndWhile
        \State $M \gets \{\}$
        \State $c_2 \gets 0$
        \While{$c_2 < K$}
        \State $c_1 \gets 0$
        \While{$c_1 < c_2$}
        \If{$Sim[c_1, c_2] > th_{merge}$}
        \State $M[c_2] \gets c_1$
        \State break
        \EndIf
        \State $c_1 \gets c_1 + 1$  
        \EndWhile
        \State $c_2 \gets c_2 + 1$  
        \EndWhile
        
        \algstore{bkbreak}
       
    \end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
    \begin{algorithmic}
        \algrestore{bkbreak}
        \State $c_1 \gets 0$
        \While{$c_1 < K$}
        \State $key \gets K-c_1-1$
        \If{$key$ in $M$.$keys$}
        \State $labels[labels = key] \gets M[key]$
        \EndIf
        \State $c_1 \gets c_1 + 1$  
        \EndWhile
        \State $labels \gets$ split($labels$, cumsum($[H\times W] * N$))
        \State $votes \gets [0] * K$
        \State $idx \gets 0$
        \While{$idx < N$}
        \State $label \gets 0$
        \While{$label < K$}
        \State $lsal \gets saliency[labels[idx][:, 0] = label]$.mean
        \If{$lsal > th_{sal}$}
        \State $votes[label] \gets votes[label] + 1$
        \EndIf
        \State $label \gets label + 1$
        \EndWhile
        \State $idx \gets idx + 1$
        \EndWhile
        \State $S \gets range(K)[votes \geq \lceil N * \frac{percentage}{100} \rceil]$
    \end{algorithmic}
\end{algorithm}

==> alg/alg_pyramid.tex <==
\begin{algorithm*}[t]
    \caption{\textbf{Pyramid Construction Algorithm.} Get an RGB image ($H \times W \times 3$). $H$ and $W$ are image height and width. Get extractor that takes in tensor $B \times 3 \times h' \times w'$ and output another tensor $B \times D \times h \times w$.}
    \label{alg:pyr_final}
    \begin{algorithmic}
        \Require $image \in R^{H \times W \times 3}$,  $extractor \gets dino\_vit8$
        \State $N_{samples} \gets [0, 0.5, 1]$
        \State $lsize \gets 128$
        \Ensure $F \in R^{1 \times D \times H \times W}$
        \State $H, W, \gets image$.shape[:2]
        \State $dH \gets H$
        \State $dW \gets \lfloor\frac{lsize}{H} \times W \rfloor$
        \State $F \gets$ None
        \State $counter \gets$ None
        \State $image \gets image$.permute($2, 0, 1$)[None, ...]
        \State $idx \gets 0$
        \While{$idx < $len($N_{samples}$)}
        \State $N \gets N_{samples}$[$idx$]
        \If{$N = 0$}
        \State $batch \gets $ Interpolate($image$, ($dH$, $dW$))
        \State $raw \gets extractor$($batch$) 
        \State $F \gets $ Interpolate($raw$, ($H$,$W$))
        \State $counter \gets$ Ones($1 \times 1 \times H \times W$)
        \Else
        \State $sH \gets 0$
        \While{$sH < H - \lfloor \frac{dH}{N} \rfloor$}
        \State $sW \gets 0$
        \While{$sW < W - \lfloor \frac{dW}{N} \rfloor$}
        \State $batch \gets $ $image$[:, :, $sH$:$sH$+$\lfloor \frac{dH}{N} \rfloor$, $sW$:$sW$+$\lfloor \frac{dW}{N} \rfloor$]
        \State $batch \gets $ Interpolate($batch$, ($dH$, $dW$))
        \State $raw \gets extractor$($batch$) 
        \State $raw \gets $Interpolate($raw$, ($\lfloor\frac{dH}{N}\rfloor$,$\lfloor\frac{dW}{N}\rfloor$))
        \State $F$[:, :, $sH$:$sH$+$\lfloor \frac{dH}{N} \rfloor$, $sW$:$sW$+$\lfloor \frac{dW}{N} \rfloor$]  += $raw$
        \State $counter$[:, :, $sH$:$sH$+$\lfloor \frac{dH}{N} \rfloor$, $sW$:$sW$+$\lfloor \frac{dW}{N} \rfloor$]  += $1$
        \State $sW = $min($W - \lfloor\frac{dW}{N}\rfloor - 1$, $sW + \lfloor\frac{\lfloor\frac{dW}{N}\rfloor}{2}\rfloor$)
        \EndWhile
        \State $sH = $min($H - \lfloor\frac{dH}{N}\rfloor - 1$, $sH + \lfloor\frac{\lfloor\frac{dH}{N}\rfloor}{2}\rfloor$)
        \EndWhile
        \EndIf
        \State $idx \gets idx + 1$
        \EndWhile
        \State $F \gets F / (1e^{-16} + counter)$
        
    \end{algorithmic}
\end{algorithm*}

==> alg/alg_pyramid_new.tex <==
\begin{algorithm*}[t]
    \caption{\textbf{Pyramid Construction Algorithm (Example).} Given an RGB image $I$ of size ($H \times W \times 3$) and a $D$-dimensional feature extractor $E : (A \times B \times 3) \mapsto (\nicefrac{A}{4} \times \nicefrac{B}{4} \times D)$, produce a processed feature map for the input image.}
    \label{alg:pyr_final}
    \begin{algorithmic}
        \Require $I \in R^{H \times W \times 3}$,  $E \gets dino\_vit8$, $H$, $W$, $D$
        \State $level0 \gets I$
        \State $level1 \gets \textsc{downsample}(I, 480, 256)$ \Comment{Downsample image to 480 $
        \times$ 256.}
        \State $level2 \gets \textsc{downsample}(I, 240, 128)$
        \State $all\_patches\_in\_imagespace \gets []$
        \For{$level \in [level0, level1, level2]$}
        \State $x \gets 0$
        \While{$x + 240 \leq W$}
        \State $y \gets 0$
        \While{$y + 128 \leq H$}
        \State $patch \gets level[y:y+128,x:x+240,:]$
        \State $feature\_patch \gets \textsc{upsample}(E(patch), 240, 128)$
        \State $patch\_in\_imagespace \gets \textsc{new\_null\_array}(H, W, D)$  \Comment{To hold features in their input image location.}
        \State $patch\_in\_imagespace[y:y+128,x:x+240,:] \gets feature\_patch$
        \State $all\_patches\_in\_imagespace.\textsc{append}(patch\_in\_imagespace)$
        \State $y \gets y + 64$
        \EndWhile
        \State $x \gets x + 64$
        \EndWhile
        \EndFor
        \State $output\_full \gets \textsc{non\_null\_average}(all\_patches\_in\_imagespace)$ \Comment{Element-wise average of non-null values.}
        \State $output \gets \textsc{pca}(output\_full, 64)$
        
    \end{algorithmic}
\end{algorithm*}

==> fig/fig_3D_noise/fig_3D_noise.tex <==
{
\begin{figure}[t]
    \centering
    \setlength{\tabcolsep}{1pt}
    
    % Set figure images paths for sequences
    % \newcommand{\figSeqJumping}{fig/fig_foreground/jumping}
    \newcommand{\figSeqBalloon}{fig/fig_anno/balloon}
    \newcommand{\figSeqBalloonw}{fig/fig_anno/balloon2}
    \newcommand{\figSeqDynamicFace}{fig/fig_anno/dynamicFace}
    \newcommand{\figSeqJumping}{fig/fig_anno/jumping}
    \newcommand{\figSeqSkating}{fig/fig_anno/skating}
    \newcommand{\figSeqPlayground}{fig/fig_anno/playground}
    \newcommand{\figSeqTruck}{fig/fig_anno/truck}
    \newcommand{\figSeqUmbrella}{fig/fig_anno/umbrella}

    % Set color remapping (can brighten images this way)
    \newcommand{\graymap}{{0 1}}
    \newcommand{\graymapBrighter}{{0.2 1.2}}
    \newcommand{\rgbcolormap}{{0 1 0 1 0 1}}
    \newcommand{\rgbcolormapFlip}{{0 1 0 1 0 1}}
    \newcommand{\rgbcolormapBrighter}{{1 0 1 0 1 0}}
    

    % Set image size
    \newcommand{\imgw}{0.49\linewidth} % 5-across figure
    \newcommand{\imgwhalf}{0.249\linewidth} % 5-across half-width figure
    %\newcommand{\imgh}{1in}
    
    % Command to draw an image with a different color map + crop as needed
    \newcommand{\imgRGB}[2][0px 0px 0px 0px]{\includegraphics[draft=\isdraft,width=\imgw,trim=#1,clip]{#2}}
    
    \newcommand{\imgAtt}[2][0px 0px 0px 0px]{\includegraphics[draft=\isdraft,decodearray={0.2 1.2},width=\imgw,trim=#1,clip]{#2}}

    \newcommand{\imgAttBr}[2][0px 0px 0px 0px]{\includegraphics[draft=\isdraft,decodearray={0.2 1.4},width=\imgw,trim=#1,clip]{#2}}

    % ^^^ NOTE DRAFT COMMAND!
    % Uncomment to actually show the pictures
    % ^^^

    \newcommand{\zoomRGB}[4]{
        \begin{tikzpicture}[
    		image/.style={inner sep=0pt, outer sep=0pt},
    		collabel/.style={above=9pt, anchor=north, inner ysep=0pt, align=center}, % scale=0.8
    		rowlabel/.style={left=9pt, rotate=90, anchor=north, inner ysep=0pt, scale=0.8, align=center},
    		subcaption/.style={inner xsep=0.75mm, inner ysep=0.75mm, below right},
    		arrow/.style={-{Latex[length=2.5mm,width=4mm]}, line width=2mm},
    		spy using outlines={rectangle, size=1.25cm, magnification=3, connect spies, ultra thick, every spy on node/.append style={thick}},
    		style1/.style={cyan!90!black,thick},
    		style2/.style={orange!90!black},
    		style3/.style={blue!90!black},
    		style4/.style={green!90!black},
    		style5/.style={white},
    		style6/.style={black},
        ]
        
        \node [image] (#1) {\imgRGB[100px 0px 0px 0px]{#2}};
        \spy[style5] on ($(#1.center)-#3$) in node (crop-#1) [anchor=#4] at (#1.#4);
        
        \end{tikzpicture}
    }

    \newcommand{\zoomAtt}[4]{
        \begin{tikzpicture}[
    		image/.style={inner sep=0pt, outer sep=0pt},
    		collabel/.style={above=9pt, anchor=north, inner ysep=0pt, align=center}, % scale=0.8
    		rowlabel/.style={left=9pt, rotate=90, anchor=north, inner ysep=0pt, scale=0.8, align=center},
    		subcaption/.style={inner xsep=0.75mm, inner ysep=0.75mm, below right},
    		arrow/.style={-{Latex[length=2.5mm,width=4mm]}, line width=2mm},
    		spy using outlines={rectangle, size=1.25cm, magnification=3, connect spies, ultra thick, every spy on node/.append style={thick}},
    		style1/.style={cyan!90!black,thick},
    		style2/.style={orange!90!black},
    		style3/.style={blue!90!black},
    		style4/.style={green!90!black},
    		style5/.style={white},
    		style6/.style={black},
        ]
        
        \node [image] (#1) {\imgAtt[100px 0px 0px 0px]{#2}};
        \spy[style5] on ($(#1.center)-#3$) in node (crop-#1) [anchor=#4] at (#1.#4);
        
        \end{tikzpicture}
    }

    \newcommand{\zoomAttBr}[4]{
        \begin{tikzpicture}[
    		image/.style={inner sep=0pt, outer sep=0pt},
    		collabel/.style={above=9pt, anchor=north, inner ysep=0pt, align=center}, % scale=0.8
    		rowlabel/.style={left=9pt, rotate=90, anchor=north, inner ysep=0pt, scale=0.8, align=center},
    		subcaption/.style={inner xsep=0.75mm, inner ysep=0.75mm, below right},
    		arrow/.style={-{Latex[length=2.5mm,width=4mm]}, line width=2mm},
    		spy using outlines={rectangle, size=1.25cm, magnification=3, connect spies, ultra thick, every spy on node/.append style={thick}},
    		style1/.style={cyan!90!black,thick},
    		style2/.style={orange!90!black},
    		style3/.style={blue!90!black},
    		style4/.style={green!90!black},
    		style5/.style={white},
    		style6/.style={black},
        ]
        
        \node [image] (#1) {\imgAttBr[100px 0px 0px 0px]{#2}};
        \spy[style5] on ($(#1.center)-#3$) in node (crop-#1) [anchor=#4] at (#1.#4);
        
        \end{tikzpicture}
    }

    \scriptsize
    \begin{tabular}{c c}
    
    % Legend.
    % Note: first column is rotated sequence title


     
    %%%%%%%%%%%%%%%%%%%%%%%%%
    % Sequence: Features

    % Labels
    Training View &
    3D Side View
    \\ 
    \imgRGB[45px 50px 80px 50px]{fig/fig_3D_noise/snapshot01.png} &
    \imgRGB[90px 50px 20px 50px]{fig/fig_3D_noise/snapshot00.png}   

    \end{tabular}

    \vspace{-0.25cm}
    \caption{
        \textbf{3D samples.} Erroneous geometry reconstruction at regions invisible during training harms 3D clustering quality.
    }
    \label{fig:fig3Dnoise}
\end{figure}

}

==> fig/fig_anno/fig_anno.tex <==
{
\begin{figure*}[t]
    \centering
    \setlength{\tabcolsep}{1pt}
    
    % Set figure images paths for sequences
    % \newcommand{\figSeqJumping}{fig/fig_foreground/jumping}
    \newcommand{\figSeqBalloon}{fig/fig_anno/balloon}
    \newcommand{\figSeqBalloonw}{fig/fig_anno/balloon2}
    \newcommand{\figSeqDynamicFace}{fig/fig_anno/dynamicFace}
    \newcommand{\figSeqJumping}{fig/fig_anno/jumping}
    \newcommand{\figSeqSkating}{fig/fig_anno/skating}
    \newcommand{\figSeqPlayground}{fig/fig_anno/playground}
    \newcommand{\figSeqTruck}{fig/fig_anno/truck}
    \newcommand{\figSeqUmbrella}{fig/fig_anno/umbrella}

    % Set color remapping (can brighten images this way)
    \newcommand{\graymap}{{0 1}}
    \newcommand{\graymapBrighter}{{0.2 1.2}}
    \newcommand{\rgbcolormap}{{0 1 0 1 0 1}}
    \newcommand{\rgbcolormapFlip}{{0 1 0 1 0 1}}
    \newcommand{\rgbcolormapBrighter}{{1 0 1 0 1 0}}
    

    % Set image size
    \newcommand{\imgw}{0.19\linewidth} % 5-across figure
    \newcommand{\imgwhalf}{0.095\linewidth} % 5-across half-width figure
    %\newcommand{\imgh}{1in}
    
    % Command to draw an image with a different color map + crop as needed
    \newcommand{\imgRGB}[2][0px 0px 0px 0px]{\includegraphics[draft=\isdraft,width=\imgw,trim=#1,clip]{#2}}
    
    \newcommand{\imgAtt}[2][0px 0px 0px 0px]{\includegraphics[draft=\isdraft,decodearray={0.2 1.2},width=\imgw,trim=#1,clip]{#2}}

    \newcommand{\imgAttBr}[2][0px 0px 0px 0px]{\includegraphics[draft=\isdraft,decodearray={0.2 1.4},width=\imgw,trim=#1,clip]{#2}}

    % ^^^ NOTE DRAFT COMMAND!
    % Uncomment to actually show the pictures
    % ^^^

    \newcommand{\zoomRGB}[4]{
        \begin{tikzpicture}[
    		image/.style={inner sep=0pt, outer sep=0pt},
    		collabel/.style={above=9pt, anchor=north, inner ysep=0pt, align=center}, % scale=0.8
    		rowlabel/.style={left=9pt, rotate=90, anchor=north, inner ysep=0pt, scale=0.8, align=center},
    		subcaption/.style={inner xsep=0.75mm, inner ysep=0.75mm, below right},
    		arrow/.style={-{Latex[length=2.5mm,width=4mm]}, line width=2mm},
    		spy using outlines={rectangle, size=1.25cm, magnification=3, connect spies, ultra thick, every spy on node/.append style={thick}},
    		style1/.style={cyan!90!black,thick},
    		style2/.style={orange!90!black},
    		style3/.style={blue!90!black},
    		style4/.style={green!90!black},
    		style5/.style={white},
    		style6/.style={black},
        ]
        
        \node [image] (#1) {\imgRGB[100px 0px 0px 0px]{#2}};
        \spy[style5] on ($(#1.center)-#3$) in node (crop-#1) [anchor=#4] at (#1.#4);
        
        \end{tikzpicture}
    }

    \newcommand{\zoomAtt}[4]{
        \begin{tikzpicture}[
    		image/.style={inner sep=0pt, outer sep=0pt},
    		collabel/.style={above=9pt, anchor=north, inner ysep=0pt, align=center}, % scale=0.8
    		rowlabel/.style={left=9pt, rotate=90, anchor=north, inner ysep=0pt, scale=0.8, align=center},
    		subcaption/.style={inner xsep=0.75mm, inner ysep=0.75mm, below right},
    		arrow/.style={-{Latex[length=2.5mm,width=4mm]}, line width=2mm},
    		spy using outlines={rectangle, size=1.25cm, magnification=3, connect spies, ultra thick, every spy on node/.append style={thick}},
    		style1/.style={cyan!90!black,thick},
    		style2/.style={orange!90!black},
    		style3/.style={blue!90!black},
    		style4/.style={green!90!black},
    		style5/.style={white},
    		style6/.style={black},
        ]
        
        \node [image] (#1) {\imgAtt[100px 0px 0px 0px]{#2}};
        \spy[style5] on ($(#1.center)-#3$) in node (crop-#1) [anchor=#4] at (#1.#4);
        
        \end{tikzpicture}
    }

    \newcommand{\zoomAttBr}[4]{
        \begin{tikzpicture}[
    		image/.style={inner sep=0pt, outer sep=0pt},
    		collabel/.style={above=9pt, anchor=north, inner ysep=0pt, align=center}, % scale=0.8
    		rowlabel/.style={left=9pt, rotate=90, anchor=north, inner ysep=0pt, scale=0.8, align=center},
    		subcaption/.style={inner xsep=0.75mm, inner ysep=0.75mm, below right},
    		arrow/.style={-{Latex[length=2.5mm,width=4mm]}, line width=2mm},
    		spy using outlines={rectangle, size=1.25cm, magnification=3, connect spies, ultra thick, every spy on node/.append style={thick}},
    		style1/.style={cyan!90!black,thick},
    		style2/.style={orange!90!black},
    		style3/.style={blue!90!black},
    		style4/.style={green!90!black},
    		style5/.style={white},
    		style6/.style={black},
        ]
        
        \node [image] (#1) {\imgAttBr[100px 0px 0px 0px]{#2}};
        \spy[style5] on ($(#1.center)-#3$) in node (crop-#1) [anchor=#4] at (#1.#4);
        
        \end{tikzpicture}
    }

    \scriptsize
    \begin{tabular}{c c@{\hspace{0.2mm}} c@{\hspace{0.2mm}} c@{\hspace{0.2mm}} c@{\hspace{0.2mm}}  c@{\hspace{0.2mm}} c}
    
    % Legend.
    % Note: first column is rotated sequence title


     
    %%%%%%%%%%%%%%%%%%%%%%%%%
    % Sequence: Features

    % Labels
    &
    \seqBalloonNoticeBoard &
    \seqBalloonWall &
    \seqDynamicFace & 
    \seqJumping &
    \seqUmbrella
    \\    

    % Images for pyramid preprocess
    %
    \rotatebox{90}{\hspace{0.55cm} Input} &
     
    % \imgRGB[45px 0px 0px 0px]{\figSeqTwoDim/ezgif-frame-001.jpeg} &
    \imgRGB[45px 0px 0px 0px]{\figSeqBalloon/00000.png} &

    %\imgRGB[100px 0px 0px 0px]{\figSeqVolume/ezgif-frame-001-render.jpeg} &
    \imgRGB[45px 0px 0px 0px]{\figSeqBalloonw/00000.png} &

    %\imgAtt[34px 0px 0px 0px]{\figSeqTwoDim/ezgif-frame-001-sal.png} &    
    \imgRGB[45px 0px 0px 0px]{\figSeqDynamicFace/00000.png} &
    
    % \imgAtt[100px 0px 0px 0px]{\figSeqVolume/0_sal.png} 
    \imgRGB[45px 0px 0px 0px]{\figSeqJumping/00000.png} &
    
    % \imgAtt[100px 0px 0px 0px]{\figSeqVolume/0_sal.png} 
    \imgRGB[45px 0px 0px 0px]{\figSeqUmbrella/00000.png} &
    \\

    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    % Sequence: Pyramid preprocess
    
    % Labels for pyramid preprocess
    \rotatebox{90}{\hspace{0.3cm} Annotation} &
     
    % \imgRGB[45px 0px 0px 0px]{\figSeqTwoDim/ezgif-frame-001.jpeg} &
    \imgRGB[45px 0px 0px 0px]{\figSeqBalloon/training_ 0.png} &

    %\imgRGB[100px 0px 0px 0px]{\figSeqVolume/ezgif-frame-001-render.jpeg} &
    \imgRGB[45px 0px 0px 0px]{\figSeqBalloonw/training_ 0.png} &

    %\imgAtt[34px 0px 0px 0px]{\figSeqTwoDim/ezgif-frame-001-sal.png} &    
    \imgRGB[45px 0px 0px 0px]{\figSeqDynamicFace/training_ 0.png} &
    
    % \imgAtt[100px 0px 0px 0px]{\figSeqVolume/0_sal.png} 
    \imgRGB[45px 0px 0px 0px]{\figSeqJumping/training_ 0.png} &
    
    % \imgAtt[100px 0px 0px 0px]{\figSeqVolume/0_sal.png} 
    \imgRGB[45px 0px 0px 0px]{\figSeqUmbrella/training_ 0.png} &
    \\


    \end{tabular}

    \vspace{-0.25cm}
    \caption{
        \textbf{Manually annotated object masks.} Annotation masks are stored as gray-scale images.The background is assigned as pixel color $0$, and foreground instances are each labeled with a non-zero unique color. 
    }
	
    \label{fig:data annotate}
\end{figure*}

}

==> fig/fig_anno/fig_anno_rotated.tex <==
{
\begin{figure}[t]
    \centering
    \setlength{\tabcolsep}{1pt}
    
    % Set figure images paths for sequences
    % \newcommand{\figSeqJumping}{fig/fig_foreground/jumping}
    \newcommand{\figSeqBalloon}{fig/fig_anno/balloon}
    \newcommand{\figSeqBalloonw}{fig/fig_anno/balloon2}
    \newcommand{\figSeqDynamicFace}{fig/fig_anno/dynamicFace}
    \newcommand{\figSeqJumping}{fig/fig_anno/jumping}
    \newcommand{\figSeqSkating}{fig/fig_anno/skating}
    \newcommand{\figSeqPlayground}{fig/fig_anno/playground}
    \newcommand{\figSeqTruck}{fig/fig_anno/truck}
    \newcommand{\figSeqUmbrella}{fig/fig_anno/umbrella}

    % Set color remapping (can brighten images this way)
    \newcommand{\graymap}{{0 1}}
    \newcommand{\graymapBrighter}{{0.2 1.2}}
    \newcommand{\rgbcolormap}{{0 1 0 1 0 1}}
    \newcommand{\rgbcolormapFlip}{{0 1 0 1 0 1}}
    \newcommand{\rgbcolormapBrighter}{{1 0 1 0 1 0}}
    

    % Set image size
    \newcommand{\imgw}{0.49\linewidth} % 5-across figure
    \newcommand{\imgwhalf}{0.249\linewidth} % 5-across half-width figure
    %\newcommand{\imgh}{1in}
    
    % Command to draw an image with a different color map + crop as needed
    \newcommand{\imgRGB}[2][0px 0px 0px 0px]{\includegraphics[draft=\isdraft,width=\imgw,trim=#1,clip]{#2}}
    
    \newcommand{\imgAtt}[2][0px 0px 0px 0px]{\includegraphics[draft=\isdraft,decodearray={0.2 1.2},width=\imgw,trim=#1,clip]{#2}}

    \newcommand{\imgAttBr}[2][0px 0px 0px 0px]{\includegraphics[draft=\isdraft,decodearray={0.2 1.4},width=\imgw,trim=#1,clip]{#2}}

    % ^^^ NOTE DRAFT COMMAND!
    % Uncomment to actually show the pictures
    % ^^^

    \newcommand{\zoomRGB}[4]{
        \begin{tikzpicture}[
    		image/.style={inner sep=0pt, outer sep=0pt},
    		collabel/.style={above=9pt, anchor=north, inner ysep=0pt, align=center}, % scale=0.8
    		rowlabel/.style={left=9pt, rotate=90, anchor=north, inner ysep=0pt, scale=0.8, align=center},
    		subcaption/.style={inner xsep=0.75mm, inner ysep=0.75mm, below right},
    		arrow/.style={-{Latex[length=2.5mm,width=4mm]}, line width=2mm},
    		spy using outlines={rectangle, size=1.25cm, magnification=3, connect spies, ultra thick, every spy on node/.append style={thick}},
    		style1/.style={cyan!90!black,thick},
    		style2/.style={orange!90!black},
    		style3/.style={blue!90!black},
    		style4/.style={green!90!black},
    		style5/.style={white},
    		style6/.style={black},
        ]
        
        \node [image] (#1) {\imgRGB[100px 0px 0px 0px]{#2}};
        \spy[style5] on ($(#1.center)-#3$) in node (crop-#1) [anchor=#4] at (#1.#4);
        
        \end{tikzpicture}
    }

    \newcommand{\zoomAtt}[4]{
        \begin{tikzpicture}[
    		image/.style={inner sep=0pt, outer sep=0pt},
    		collabel/.style={above=9pt, anchor=north, inner ysep=0pt, align=center}, % scale=0.8
    		rowlabel/.style={left=9pt, rotate=90, anchor=north, inner ysep=0pt, scale=0.8, align=center},
    		subcaption/.style={inner xsep=0.75mm, inner ysep=0.75mm, below right},
    		arrow/.style={-{Latex[length=2.5mm,width=4mm]}, line width=2mm},
    		spy using outlines={rectangle, size=1.25cm, magnification=3, connect spies, ultra thick, every spy on node/.append style={thick}},
    		style1/.style={cyan!90!black,thick},
    		style2/.style={orange!90!black},
    		style3/.style={blue!90!black},
    		style4/.style={green!90!black},
    		style5/.style={white},
    		style6/.style={black},
        ]
        
        \node [image] (#1) {\imgAtt[100px 0px 0px 0px]{#2}};
        \spy[style5] on ($(#1.center)-#3$) in node (crop-#1) [anchor=#4] at (#1.#4);
        
        \end{tikzpicture}
    }

    \newcommand{\zoomAttBr}[4]{
        \begin{tikzpicture}[
    		image/.style={inner sep=0pt, outer sep=0pt},
    		collabel/.style={above=9pt, anchor=north, inner ysep=0pt, align=center}, % scale=0.8
    		rowlabel/.style={left=9pt, rotate=90, anchor=north, inner ysep=0pt, scale=0.8, align=center},
    		subcaption/.style={inner xsep=0.75mm, inner ysep=0.75mm, below right},
    		arrow/.style={-{Latex[length=2.5mm,width=4mm]}, line width=2mm},
    		spy using outlines={rectangle, size=1.25cm, magnification=3, connect spies, ultra thick, every spy on node/.append style={thick}},
    		style1/.style={cyan!90!black,thick},
    		style2/.style={orange!90!black},
    		style3/.style={blue!90!black},
    		style4/.style={green!90!black},
    		style5/.style={white},
    		style6/.style={black},
        ]
        
        \node [image] (#1) {\imgAttBr[100px 0px 0px 0px]{#2}};
        \spy[style5] on ($(#1.center)-#3$) in node (crop-#1) [anchor=#4] at (#1.#4);
        
        \end{tikzpicture}
    }

    \scriptsize
    \begin{tabular}{c c c}
    
    % Legend.
    % Note: first column is rotated sequence title


     
    %%%%%%%%%%%%%%%%%%%%%%%%%
    % Sequence: Features

    % Labels
    &
    Input &
    Annotation
    \\ 
    
    \rotatebox{90}{\hspace{0.3cm} \seqBalloonNoticeBoard} &
    \imgRGB[45px 0px 0px 0px]{\figSeqBalloon/00000.png} &
    \imgRGB[45px 0px 0px 0px]{\figSeqBalloon/training_ 0.png} \\

    \rotatebox{90}{\hspace{0.5cm} \seqBalloonWall} &
    \imgRGB[45px 0px 0px 0px]{\figSeqBalloonw/00000.png} &
    \imgRGB[45px 0px 0px 0px]{\figSeqBalloonw/training_ 0.png}
    \\

    \rotatebox{90}{\hspace{0.4cm} \seqDynamicFace} &
    \imgRGB[45px 0px 0px 0px]{\figSeqDynamicFace/00000.png} &
    \imgRGB[45px 0px 0px 0px]{\figSeqDynamicFace/training_ 0.png}    
    \\

    \rotatebox{90}{\hspace{0.7cm} \seqJumping} &
    \imgRGB[45px 0px 0px 0px]{\figSeqJumping/00000.png} &
    \imgRGB[45px 0px 0px 0px]{\figSeqJumping/training_ 0.png}
    \\

    \rotatebox{90}{\hspace{0.6cm} \seqUmbrella} &
    \imgRGB[45px 0px 0px 0px]{\figSeqUmbrella/00000.png} &
    \imgRGB[45px 0px 0px 0px]{\figSeqUmbrella/training_ 0.png}   

    \end{tabular}

    \vspace{-0.25cm}
    \caption{
        \textbf{Manually annotated object masks.} We store annotation masks as grayscale images. The background is assigned as pixel value $0$, and foreground instances are each assigned a unique non-zero value.
    }
    \vspace{10cm}
    \label{fig:data annotate}
\end{figure}

}

==> fig/fig_decay/fig_decay.tex <==
{
\begin{figure}[t]
    \centering
    \setlength{\tabcolsep}{1pt}
    
    % Set figure images paths for sequences
    % \newcommand{\figSeqJumping}{fig/fig_foreground/jumping}
    %\newcommand{\figSeqBalloon}{fig/fig_anno/balloon}
    \newcommand{\figSeqBalloonw}{fig/fig_decay/balloon2}
    %\newcommand{\figSeqDynamicFace}{fig/fig_post/dynamicFace}
    %\newcommand{\figSeqJumping}{fig/fig_post/jumping}
    \newcommand{\figSeqSkating}{fig/fig_decay/skating}
    %\newcommand{\figSeqPlayground}{fig/fig_anno/playground}
    %\newcommand{\figSeqTruck}{fig/fig_anno/truck}
    %\newcommand{\figSeqUmbrella}{fig/fig_anno/umbrella}

    % Set color remapping (can brighten images this way)
    \newcommand{\graymap}{{0 1}}
    \newcommand{\graymapBrighter}{{0.2 1.2}}
    \newcommand{\rgbcolormap}{{0 1 0 1 0 1}}
    \newcommand{\rgbcolormapFlip}{{0 1 0 1 0 1}}
    \newcommand{\rgbcolormapBrighter}{{1 0 1 0 1 0}}
    

    % Set image size
    \newcommand{\imgw}{0.45\linewidth} % 5-across figure
    \newcommand{\imgwhalf}{0.225\linewidth} % 5-across half-width figure
    %\newcommand{\imgh}{1in}
    
    % Command to draw an image with a different color map + crop as needed
    \newcommand{\imgRGB}[2][0px 0px 0px 0px]{\includegraphics[draft=\isdraft,width=\imgw,trim=#1,clip]{#2}}
    
    \newcommand{\imgAtt}[2][0px 0px 0px 0px]{\includegraphics[draft=\isdraft,decodearray={0.2 1.2},width=\imgw,trim=#1,clip]{#2}}

    \newcommand{\imgAttBr}[2][0px 0px 0px 0px]{\includegraphics[draft=\isdraft,decodearray={0.2 1.4},width=\imgw,trim=#1,clip]{#2}}

    % ^^^ NOTE DRAFT COMMAND!
    % Uncomment to actually show the pictures
    % ^^^

    \newcommand{\zoomRGB}[4]{
        \begin{tikzpicture}[
    		image/.style={inner sep=0pt, outer sep=0pt},
    		collabel/.style={above=9pt, anchor=north, inner ysep=0pt, align=center}, % scale=0.8
    		rowlabel/.style={left=9pt, rotate=90, anchor=north, inner ysep=0pt, scale=0.8, align=center},
    		subcaption/.style={inner xsep=0.75mm, inner ysep=0.75mm, below right},
    		arrow/.style={-{Latex[length=2.5mm,width=4mm]}, line width=2mm},
    		spy using outlines={rectangle, size=1.25cm, magnification=3, connect spies, ultra thick, every spy on node/.append style={thick}},
    		style1/.style={cyan!90!black,thick},
    		style2/.style={orange!90!black},
    		style3/.style={blue!90!black},
    		style4/.style={green!90!black},
    		style5/.style={white},
    		style6/.style={black},
        ]
        
        \node [image] (#1) {\imgRGB[45px 0px 0px 0px]{#2}};
        \spy[style5] on ($(#1.center)-#3$) in node (crop-#1) [anchor=#4] at (#1.#4);
        
        \end{tikzpicture}
    }

    \newcommand{\zoomAtt}[4]{
        \begin{tikzpicture}[
    		image/.style={inner sep=0pt, outer sep=0pt},
    		collabel/.style={above=9pt, anchor=north, inner ysep=0pt, align=center}, % scale=0.8
    		rowlabel/.style={left=9pt, rotate=90, anchor=north, inner ysep=0pt, scale=0.8, align=center},
    		subcaption/.style={inner xsep=0.75mm, inner ysep=0.75mm, below right},
    		arrow/.style={-{Latex[length=2.5mm,width=4mm]}, line width=2mm},
    		spy using outlines={rectangle, size=1.25cm, magnification=3, connect spies, ultra thick, every spy on node/.append style={thick}},
    		style1/.style={cyan!90!black,thick},
    		style2/.style={orange!90!black},
    		style3/.style={blue!90!black},
    		style4/.style={green!90!black},
    		style5/.style={white},
    		style6/.style={black},
        ]
        
        \node [image] (#1) {\imgAtt[100px 0px 0px 0px]{#2}};
        \spy[style5] on ($(#1.center)-#3$) in node (crop-#1) [anchor=#4] at (#1.#4);
        
        \end{tikzpicture}
    }

    \newcommand{\zoomAttBr}[4]{
        \begin{tikzpicture}[
    		image/.style={inner sep=0pt, outer sep=0pt},
    		collabel/.style={above=9pt, anchor=north, inner ysep=0pt, align=center}, % scale=0.8
    		rowlabel/.style={left=9pt, rotate=90, anchor=north, inner ysep=0pt, scale=0.8, align=center},
    		subcaption/.style={inner xsep=0.75mm, inner ysep=0.75mm, below right},
    		arrow/.style={-{Latex[length=2.5mm,width=4mm]}, line width=2mm},
    		spy using outlines={rectangle, size=1.25cm, magnification=3, connect spies, ultra thick, every spy on node/.append style={thick}},
    		style1/.style={cyan!90!black,thick},
    		style2/.style={orange!90!black},
    		style3/.style={blue!90!black},
    		style4/.style={green!90!black},
    		style5/.style={white},
    		style6/.style={black},
        ]
        
        \node [image] (#1) {\imgAttBr[100px 0px 0px 0px]{#2}};
        \spy[style5] on ($(#1.center)-#3$) in node (crop-#1) [anchor=#4] at (#1.#4);
        
        \end{tikzpicture}
    }

    \scriptsize
    \begin{tabular}{c c@{\hspace{0.2mm}} c@{\hspace{0.2mm}} c}
    
    % Legend.
    % Note: first column is rotated sequence title

    &
    (a) Balloon Wall &
    (b) Skating
    \\
    %%%%%%%%%%%%%%%%%%%%%%%%%
    % Sequence: Features

    % Labels
    %&
    %Balloon1-2 &
    %Balloon2-2 &
    %DynamicFace-2 & 
    %Jumping &
    %Umbrella
    %\\    

    \rotatebox{90}{Input} &

    \imgRGB[45px 0px 0px 0px]{\figSeqBalloonw/00015.png} &

    \imgRGB[45px 0px 0px 0px]{\figSeqSkating/00009.png} 
    \\


    % Images for pyramid preprocess
    %
    \rotatebox{90}{Ours+Decay} &
    
    \zoomRGB{balloon-decay}{\figSeqBalloonw/15_1.png}{(-0.2,0.4)}{north west} &

    \zoomRGB{skater-decay}{\figSeqSkating/9_1.png}{(0.9,-0.5)}{north east}
    \\

    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    % Sequence: Pyramid preprocess
    
    % Labels for pyramid preprocess
    \rotatebox{90}{Ours} &
     
    \zoomRGB{balloon-ours}{\figSeqBalloonw/15.png}{(-0.2,0.4)}{north west} &

    \zoomRGB{skater-ours}{\figSeqSkating/9.png}{(0.9,-0.5)}{north east}
    \\


    \end{tabular}

    \vspace{-0.25cm}
    \caption{
        \textbf{Decaying semantics and attention leads to missing objects and unwanted objects.} With no self-consistent constraint, the optimization is more free to adjust the meaning of regions. While this can increase edge detail, it creates worse overall results.
    }
	
    \label{fig:decay}
    \vspace{9cm}
\end{figure}

}

==> fig/fig_dycheck/fig_dycheck.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  DyCheck - Qualitative 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

{   % Scope declared variables

\begin{figure*}[t]
    \centering
    \setlength{\tabcolsep}{1pt}
    
    % Set figure images paths for sequences
    \newcommand{\figSeqHaruSit}{fig/fig_dycheck/haru-sit}
    \newcommand{\figSeqMochiHighFive}{fig/fig_dycheck/mochi-high-five}
    \newcommand{\figSeqSpaceOut}{fig/fig_dycheck/space-out}
    \newcommand{\figSeqSpin}{fig/fig_dycheck/spin}
    
    

    % Set color remapping (can brighten images this way)
    \newcommand{\rgbcolormapBrighter}{{0.2 1.2 0.2 1.2 0.2 1.2}}
    \newcommand{\rgbcolormap}{{0 1 0 1 0 1}}

    % Set image size
    \newcommand{\imgw}{0.19\linewidth}
    %\newcommand{\imgh}{0.01\linewidth}
    
    % Command to draw an image with a different color map + crop as needed
    \newcommand{\imgRGB}[2][0px 0px 0px 0px]{\includegraphics[draft=\isdraft,width=\imgw,trim=#1,clip]{#2}}

    % ^^^ NOTE DRAFT COMMAND!
    % Uncomment to actually show the pictures
    % ^^^
    
    \newcommand{\zoomRGB}[4]{
        \begin{tikzpicture}[
    		image/.style={inner sep=0pt, outer sep=0pt},
    		collabel/.style={above=9pt, anchor=north, inner ysep=0pt, align=center}, % scale=0.8
    		rowlabel/.style={left=9pt, rotate=90, anchor=north, inner ysep=0pt, scale=0.8, align=center},
    		subcaption/.style={inner xsep=0.75mm, inner ysep=0.75mm, below right},
    		arrow/.style={-{Latex[length=2.5mm,width=4mm]}, line width=2mm},
    		spy using outlines={rectangle, size=1.25cm, magnification=3, connect spies, ultra thick, every spy on node/.append style={thick}},
    		style1/.style={cyan!90!black,thick},
    		style2/.style={orange!90!black},
    		style3/.style={blue!90!black},
    		style4/.style={green!90!black},
    		style5/.style={white},
    		style6/.style={black},
        ]
        
        \node [image] (#1) {\imgRGB{#2}};
        \spy[style5] on ($(#1.center)-#3$) in node (crop-#1) [anchor=#4] at (#1.#4);
        
        \end{tikzpicture}
    }
    
    \begin{tabular}{c c@{\hspace{0.2mm}} c@{\hspace{0.2mm}} c@{\hspace{0.2mm}} c@{\hspace{0.2mm}} c}
    
    % Legend.
    % Note: first column is rotated sequence title
    & 
    (a) Input &
    (b) \semfeatnetwork (2D) & 
    (c) ProposeReduce~\cite{lin2021video} &
    (d) \titlename~(Ours; input) &
    (e) \titlename~(Ours; novel) \\
    
     %%%%%%%%%%%%%%%%%%%%%%%%%
    % Sequence: DynamicFace-2
    \rotatebox{90}{\footnotesize \seqSpaceOut} % This centers the text

    &
    \zoomRGB{balloonw-rgb-input}{\figSeqSpaceOut/00042.png}{(0.7,1.6)}{north west} &
    
    \zoomRGB{balloonw-clustering-dinovit2d}{\figSeqSpaceOut/42_DINO.png}{(0.7,1.6)}{north west} &
    
    \zoomRGB{balloonw-clustering-propred}{\figSeqSpaceOut/42_PR.png}{(0.7,1.6)}{north west} &
    
    \zoomRGB{balloonw-clustering-oursiv}{\figSeqSpaceOut/42_SAFF.png}{(0.7,1.6)}{north west} & 

    \zoomRGB{balloonw-clustering-oursnv}{\figSeqSpaceOut/35_SAFF.png}{(0.3, 1.6)}{north east} 
    \\[-1pt]

    
    
    %%%%%%%%%%%%%%%%%%%%%%%%%
    % Sequence: Balloon 1 (Notice Board)
    \rotatebox{90}{\footnotesize \seqSpin (person is cross-legged)} % This centers the text

    &
    \zoomRGB{balloonw-rgb-input}{\figSeqSpin/00014.png}{(0.1,0.3)}{north west} &
    
    \zoomRGB{balloonw-clustering-dinovit2d}{\figSeqSpin/14_DINO.png}{(0.1,0.3)}{north west} &
    
    \zoomRGB{balloonw-clustering-propred}{\figSeqSpin/14_PR.png}{(0.1,0.3)}{north west} &
    
    \zoomRGB{balloonw-clustering-oursiv}{\figSeqSpin/14_SAFF.png}{(0.1,0.3)}{north west} & 

    \zoomRGB{balloonw-clustering-oursnv}{\figSeqSpin/92_SAFF.png}{(1.5,0.05)}{north east} 
    \\[-1pt]
    %%%%%%%%%%%%%%%%%%%%%%%%%

    \end{tabular}

    \vspace{-0.25cm}
    \caption{
        \textbf{\titlename can apply to \dycheck.}
        For monocular casually-captured data, \titlename produces significantly better detail than raw \semfeatnetwork and is comparable to supervised large-scale 2D video learning~\cite{lin2021video}. Some fine details are improved (\seqSpin, fingers) and novel views maintain their geometry (\seqSpin, gap between legs occluded by head at input timestep).
    }
    \label{fig:dycheck}
    \vspace{-0.25cm}
\end{figure*}

}

==> fig/fig_edits/fig_edits.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  Scene editing figure
% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

{   % Scope declared variables

\begin{figure}[t]
    \centering
    \setlength{\tabcolsep}{1pt}
    
    % Set figure images paths for sequences
    \newcommand{\figEdits}{fig/fig_edits}
    %\newcommand{\figSeqFg}{fig/fig_merge/Fg}

    % Set color remapping (can brighten images this way)
    \newcommand{\graymap}{{0 1}}
    \newcommand{\graymapBrighter}{{0.2 1.2}}
    \newcommand{\rgbcolormap}{{0 1 0 1 0 1}}
    \newcommand{\rgbcolormapBrighter}{{1 0 1 0 1 0}}
    
    % Set image size
    \newcommand{\imgw}{0.49\linewidth} % 4-across figure
    %\newcommand{\imgh}{1in}
    
    % Command to draw an image with a different color map + crop as needed
    \newcommand{\imgRGB}[2][0px 0px 100px 0px]{\includegraphics[draft=\isdraft,width=\imgw,trim=#1,clip]{#2}}

    % ^^^ NOTE DRAFT COMMAND!
    % Uncomment to actually show the pictures
    % ^^^
    \scriptsize
    %\begin{tabular}{c | c@{\hspace{0.2mm}} c@{\hspace{0.2mm}} c@{\hspace{0.2mm}}}
    \begin{tabular}{c c}
    
    %%%%%%%%%%%%%%%%%%%%%%%%%
    % First row
    
    %%%%%
    % Labels
    (a) Novel SAFF RGB output &
    (b) Depth of field
    \\    

    %%%%%
    % Images
    % Input
    \imgRGB{\figEdits/input.png} &
    % Semantics
    \imgRGB{\figEdits/dof.png}
    \\

    %%%%%%%%%%%%%%%%%%%%%%%%%
    % Second row

    %%%%%
    % Labels
    
    % Empty space
    (c) Darkened background &
    (d) Color adjustment
    \\
    \imgRGB{\figEdits/dark.png} &
    
    \imgRGB{\figEdits/color.png}

    \end{tabular}

    \vspace{-0.25cm}
    \caption{
        \textbf{Decomposition enables scene editing.} Using the scene decomposition from SAFF, we are able to apply visual effects that automatically highlight or target the salient objects in the scene, even when rendering novel views.
    }
	
    \label{fig:edits}
    \vspace{-0.25cm}
\end{figure}

}

==> fig/fig_feature_extraction/fig_feature_extraction.tex <==

\begin{figure}
    \centering
    %\includegraphics{fig/dinoe.pdf}
    \missingfigure{Pyramid dino extraction}
    \caption{Pyramid 
    DINO Extraction. \url{https://docs.google.com/drawings/d/1UrGxtQVXffpxsUUmw9Fli7xuESK6RKuiKcoBrMZp-_8/edit?usp=sharing}
    }
    \label{fig:feature_extraction}
\end{figure}

==> fig/fig_kidrunning/fig_kidrunning.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  KidRunning 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

{   % Scope declared variables

\begin{figure*}[t]
    \centering
    %\setlength{\tabcolsep}{1pt}
    
    % Set figure images paths for sequences
    \newcommand{\figSeqKid}{fig/fig_kidrunning}
    

    % Set color remapping (can brighten images this way)
    \newcommand{\rgbcolormapBrighter}{{0.2 1.2 0.2 1.2 0.2 1.2}}
    \newcommand{\rgbcolormap}{{0 1 0 1 0 1}}

    % Set image size
    \newcommand{\imgw}{0.22\linewidth}
    %\newcommand{\imgh}{0.01\linewidth}
    
    % Command to draw an image with a different color map + crop as needed
    \newcommand{\imgRGB}[2][0px 0px 0px 0px]{\includegraphics[draft=\isdraft,width=\imgw,trim=#1,clip]{#2}}

    % ^^^ NOTE DRAFT COMMAND!
    % Uncomment to actually show the pictures
    % ^^^
    
    \newcommand{\zoomRGB}[4]{
        \begin{tikzpicture}[
    		image/.style={inner sep=0pt, outer sep=0pt},
    		collabel/.style={above=9pt, anchor=north, inner ysep=0pt, align=center}, % scale=0.8
    		rowlabel/.style={left=9pt, rotate=90, anchor=north, inner ysep=0pt, scale=0.8, align=center},
    		subcaption/.style={inner xsep=0.75mm, inner ysep=0.75mm, below right},
    		arrow/.style={-{Latex[length=2.5mm,width=4mm]}, line width=2mm},
    		spy using outlines={rectangle, size=1.25cm, magnification=3, connect spies, ultra thick, every spy on node/.append style={thick}},
    		style1/.style={cyan!90!black,thick},
    		style2/.style={orange!90!black},
    		style3/.style={blue!90!black},
    		style4/.style={green!90!black},
    		style5/.style={white},
    		style6/.style={black},
        ]
        
        \node [image] (#1) {\imgRGB{#2}};
        \spy[style5] on ($(#1.center)-#3$) in node (crop-#1) [anchor=#4] at (#1.#4);
        
        \end{tikzpicture}
    }
    
    \begin{tabular}{c c@{\hspace{0.2mm}} c@{\hspace{0.2mm}} c@{\hspace{0.2mm}} c@{\hspace{0.2mm}} c}
    
    % Legend.
    % Note: first column is rotated sequence title
    & 
    (a) Ground Truth &
    (b) RGB Rendering & 
    (c) Depth Rendering &
    (d) Decomposition  \\
    
     %%%%%%%%%%%%%%%%%%%%%%%%%
    % Sequence: DynamicFace-2
    \rotatebox{90}{\footnotesize \datasplitInput} % This centers the text

    &
    \imgRGB[45px 0px 90px 0px]{\figSeqKid/00043.png}
     &
    
     \imgRGB[45px 0px 90px 0px]{\figSeqKid/43_rgb.png}&
    
     \imgRGB[45px 0px 90px 0px]{\figSeqKid/43_depth.png} &
    
    \imgRGB[45px 0px 90px 0px]{\figSeqKid/43_cluster.png}

    \\[-1pt]

    
    
    %%%%%%%%%%%%%%%%%%%%%%%%%
    % Sequence: Balloon 1 (Notice Board)
    \rotatebox{90}{\footnotesize \datasplitTest} % This centers the text

    &
     \imgRGB[45px 0px 90px 0px]{\figSeqKid/00026.png} &
    
     \imgRGB[45px 0px 90px 0px]{\figSeqKid/26_rgb.png} &
    
     \imgRGB[45px 0px 90px 0px]{\figSeqKid/26_depth.png} &
    
     \imgRGB[45px 0px 90px 0px]{\figSeqKid/26_cluster.png} 

    \\[-1pt]

   
     %%%%%%%%%%%%%%%%%%%%%%%%%
    

   
    
    
    %%%%%%%%%%%%%%%%%%%%%%%%%
   
    %%%%%%%%%%%%%%%%%%%%%%%%%
    % Sequence: xxx

    % In general, we will pick a small set of sequences that show off key properties of our method.

    \end{tabular}

    \vspace{-0.25cm}
    \caption{
        \titlename's rendering and decomposition result on the \emph{kid-running} scene.
    }
    \label{fig:kid_running}
\end{figure*}

}

==> fig/fig_movi/fig_movi.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  MOVI Comparison
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

{   % Scope declared variables

\begin{figure}[t]
    \centering
    \setlength{\tabcolsep}{1pt}
    
    % Set figure images paths for sequences
    \newcommand{\figSeqBasket}{fig/fig_movi/basket}
    \newcommand{\figSeqPinkShoe}{fig/fig_movi/pinkshoe}

    % Set color remapping (can brighten images this way)
    \newcommand{\rgbcolormapBrighter}{{0.2 1.2 0.2 1.2 0.2 1.2}}
    \newcommand{\rgbcolormap}{{0 1 0 1 0 1}}

    % Set image size
    \newcommand{\imgw}{1.08in}
    \newcommand{\imgh}{1.08in}
    
    % Command to draw an image with a different color map + crop as needed
    \newcommand{\imgRGB}[2][0px 0px 0px 0px]{\includegraphics[draft=\isdraft,decodearray=\rgbcolormap,width=\imgw,height=\imgh,trim=#1,clip]{#2}}
    
    
   
    % ^^^ NOTE DRAFT COMMAND!
    % Uncomment to actually show the pictures
    % ^^^
    
    \begin{tabular}{c c@{\hspace{0.2mm}} c@{\hspace{0.2mm}} c@{\hspace{0.2mm}} c@{\hspace{0.2mm}} c}
    
    % Legend.
    % Note: first column is rotated sequence title
    & 
    (a) Input &
    (b) SAVI++\cite{elsayed2022savipp} &
    (c) \titlename~(Ours) & \\

    %%%%%%%%%%%%%%%%%%%%%%%%%
    % Sequence: Basket
    &
    \includegraphics[width=\imgw,height=\imgh]{\figSeqBasket/input.png} &
    
    \includegraphics[width=\imgw,height=\imgh]{\figSeqBasket/savi.png} &
    
    \includegraphics[width=\imgw,height=\imgh]{\figSeqBasket/ours.png} &
    \\[-1pt]


    %%%%%%%%%%%%%%%%%%%%%%%%%
    % Sequence: Pink shoe
    &
    \includegraphics[width=\imgw,height=\imgh]{\figSeqPinkShoe/input.png} &
    
    \includegraphics[width=\imgw,height=\imgh]{\figSeqPinkShoe/savi.png} &
    
    \includegraphics[width=\imgw,height=\imgh]{\figSeqPinkShoe/ours.png} &
    \\[-1pt]


    %%%%%%%%%%%%%%%%%%%%%%%%%
    % Sequence: xxx

    % In general, we will pick a small set of sequences that show off key properties of our method.

    \end{tabular}

    \vspace{-0.25cm}
    \caption{
        \textbf{Saliency-aware clustering improves semantic decomposition on synthetic sequences.}
        Compared to SAVI++ \cite{elsayed2022savipp}, a baseline that is trained using labeled synthetic sequences, our method produces cleaner foreground/background boundaries and more clearly discovers all objects in the scene. These sequences are from the MOVI-E dataset \cite{greff2021kubric}. \el{We may axe the SAVI comparison but figured I'd take a stab at it in case we want it. Could also make a claim about our ability to cluster from novel views?}
    }
	
    \label{fig:movi}
\end{figure}

}

==> fig/fig_post/fig_post.tex <==
{
\begin{figure}[t]
    \centering
    \setlength{\tabcolsep}{1pt}
    
    % Set figure images paths for sequences
    % \newcommand{\figSeqJumping}{fig/fig_foreground/jumping}
    %\newcommand{\figSeqBalloon}{fig/fig_anno/balloon}
    %\newcommand{\figSeqBalloonw}{fig/fig_anno/balloon2}
    \newcommand{\figSeqDynamicFace}{fig/fig_post/dynamicFace}
    \newcommand{\figSeqJumping}{fig/fig_post/jumping}
    %\newcommand{\figSeqSkating}{fig/fig_anno/skating}
    %\newcommand{\figSeqPlayground}{fig/fig_anno/playground}
    %\newcommand{\figSeqTruck}{fig/fig_anno/truck}
    %\newcommand{\figSeqUmbrella}{fig/fig_anno/umbrella}

    % Set color remapping (can brighten images this way)
    \newcommand{\graymap}{{0 1}}
    \newcommand{\graymapBrighter}{{0.2 1.2}}
    \newcommand{\rgbcolormap}{{0 1 0 1 0 1}}
    \newcommand{\rgbcolormapFlip}{{0 1 0 1 0 1}}
    \newcommand{\rgbcolormapBrighter}{{1 0 1 0 1 0}}
    

    % Set image size
    \newcommand{\imgw}{0.47\linewidth} % 5-across figure
    \newcommand{\imgwhalf}{0.225\linewidth} % 5-across half-width figure
    %\newcommand{\imgh}{1in}
    
    % Command to draw an image with a different color map + crop as needed
    \newcommand{\imgRGB}[2][0px 0px 0px 0px]{\includegraphics[draft=\isdraft,width=\imgw,trim=#1,clip]{#2}}
    
    \newcommand{\imgAtt}[2][0px 0px 0px 0px]{\includegraphics[draft=\isdraft,decodearray={0.2 1.2},width=\imgw,trim=#1,clip]{#2}}

    \newcommand{\imgAttBr}[2][0px 0px 0px 0px]{\includegraphics[draft=\isdraft,decodearray={0.2 1.4},width=\imgw,trim=#1,clip]{#2}}

    % ^^^ NOTE DRAFT COMMAND!
    % Uncomment to actually show the pictures
    % ^^^

    \newcommand{\zoomRGB}[4]{
        \begin{tikzpicture}[
    		image/.style={inner sep=0pt, outer sep=0pt},
    		collabel/.style={above=9pt, anchor=north, inner ysep=0pt, align=center}, % scale=0.8
    		rowlabel/.style={left=9pt, rotate=90, anchor=north, inner ysep=0pt, scale=0.8, align=center},
    		subcaption/.style={inner xsep=0.75mm, inner ysep=0.75mm, below right},
    		arrow/.style={-{Latex[length=2.5mm,width=4mm]}, line width=2mm},
    		spy using outlines={rectangle, size=1.25cm, magnification=3, connect spies, ultra thick, every spy on node/.append style={thick}},
    		style1/.style={cyan!90!black,thick},
    		style2/.style={orange!90!black},
    		style3/.style={blue!90!black},
    		style4/.style={green!90!black},
    		style5/.style={white},
    		style6/.style={black},
        ]
        
        \node [image] (#1) {\imgRGB[100px 0px 0px 0px]{#2}};
        \spy[style5] on ($(#1.center)-#3$) in node (crop-#1) [anchor=#4] at (#1.#4);
        
        \end{tikzpicture}
    }

    \newcommand{\zoomAtt}[4]{
        \begin{tikzpicture}[
    		image/.style={inner sep=0pt, outer sep=0pt},
    		collabel/.style={above=9pt, anchor=north, inner ysep=0pt, align=center}, % scale=0.8
    		rowlabel/.style={left=9pt, rotate=90, anchor=north, inner ysep=0pt, scale=0.8, align=center},
    		subcaption/.style={inner xsep=0.75mm, inner ysep=0.75mm, below right},
    		arrow/.style={-{Latex[length=2.5mm,width=4mm]}, line width=2mm},
    		spy using outlines={rectangle, size=1.25cm, magnification=3, connect spies, ultra thick, every spy on node/.append style={thick}},
    		style1/.style={cyan!90!black,thick},
    		style2/.style={orange!90!black},
    		style3/.style={blue!90!black},
    		style4/.style={green!90!black},
    		style5/.style={white},
    		style6/.style={black},
        ]
        
        \node [image] (#1) {\imgAtt[100px 0px 0px 0px]{#2}};
        \spy[style5] on ($(#1.center)-#3$) in node (crop-#1) [anchor=#4] at (#1.#4);
        
        \end{tikzpicture}
    }

    \newcommand{\zoomAttBr}[4]{
        \begin{tikzpicture}[
    		image/.style={inner sep=0pt, outer sep=0pt},
    		collabel/.style={above=9pt, anchor=north, inner ysep=0pt, align=center}, % scale=0.8
    		rowlabel/.style={left=9pt, rotate=90, anchor=north, inner ysep=0pt, scale=0.8, align=center},
    		subcaption/.style={inner xsep=0.75mm, inner ysep=0.75mm, below right},
    		arrow/.style={-{Latex[length=2.5mm,width=4mm]}, line width=2mm},
    		spy using outlines={rectangle, size=1.25cm, magnification=3, connect spies, ultra thick, every spy on node/.append style={thick}},
    		style1/.style={cyan!90!black,thick},
    		style2/.style={orange!90!black},
    		style3/.style={blue!90!black},
    		style4/.style={green!90!black},
    		style5/.style={white},
    		style6/.style={black},
        ]
        
        \node [image] (#1) {\imgAttBr[100px 0px 0px 0px]{#2}};
        \spy[style5] on ($(#1.center)-#3$) in node (crop-#1) [anchor=#4] at (#1.#4);
        
        \end{tikzpicture}
    }

    \scriptsize
    \begin{tabular}{c c@{\hspace{0.2mm}} c@{\hspace{0.2mm}} c}
    
    % Legend.
    % Note: first column is rotated sequence title

    &
    \seqDynamicFace &
    \seqJumping
    \\
    %%%%%%%%%%%%%%%%%%%%%%%%%
    % Sequence: Features

    % Labels
    %&
    %Balloon1-2 &
    %Balloon2-2 &
    %DynamicFace-2 & 
    %Jumping &
    %Umbrella
    %\\    

    \rotatebox{90}{\hspace{0.6cm} Input} &
     
    % \imgRGB[45px 0px 0px 0px]{\figSeqTwoDim/ezgif-frame-001.jpeg} &
    %\imgRGB[45px 0px 0px 0px]{\figSeqBalloon/00000.png} &

    %\imgRGB[100px 0px 0px 0px]{\figSeqVolume/ezgif-frame-001-render.jpeg} &
    %\imgRGB[45px 0px 0px 0px]{\figSeqBalloonw/00000.png} &

    %\imgAtt[34px 0px 0px 0px]{\figSeqTwoDim/ezgif-frame-001-sal.png} &    
    \imgRGB[45px 0px 0px 0px]{\figSeqDynamicFace/00015.png} &
    
    % \imgAtt[100px 0px 0px 0px]{\figSeqVolume/0_sal.png} 
    \imgRGB[45px 0px 0px 0px]{\figSeqJumping/00023.png} &
    
    % \imgAtt[100px 0px 0px 0px]{\figSeqVolume/0_sal.png} 
    %\imgRGB[45px 0px 0px 0px]{\figSeqUmbrella/00000.png} &
    \\


    % Images for pyramid preprocess
    %
    \rotatebox{90}{\hspace{0.7cm} Raw} &
     
    % \imgRGB[45px 0px 0px 0px]{\figSeqTwoDim/ezgif-frame-001.jpeg} &
    %\imgRGB[45px 0px 0px 0px]{\figSeqBalloon/00000.png} &

    %\imgRGB[100px 0px 0px 0px]{\figSeqVolume/ezgif-frame-001-render.jpeg} &
    %\imgRGB[45px 0px 0px 0px]{\figSeqBalloonw/00000.png} &

    %\imgAtt[34px 0px 0px 0px]{\figSeqTwoDim/ezgif-frame-001-sal.png} &    
    \imgRGB[45px 0px 0px 0px]{\figSeqDynamicFace/15_raw.png} &
    
    % \imgAtt[100px 0px 0px 0px]{\figSeqVolume/0_sal.png} 
    \imgRGB[45px 0px 0px 0px]{\figSeqJumping/23_raw.png} &
    
    % \imgAtt[100px 0px 0px 0px]{\figSeqVolume/0_sal.png} 
    %\imgRGB[45px 0px 0px 0px]{\figSeqUmbrella/00000.png} &
    \\

    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    % Sequence: Pyramid preprocess
    
    % Labels for pyramid preprocess
    \rotatebox{90}{\hspace{0.3cm} Post Processed} &
     
    % \imgRGB[45px 0px 0px 0px]{\figSeqTwoDim/ezgif-frame-001.jpeg} &
    %\imgRGB[45px 0px 0px 0px]{\figSeqBalloon/training_ 0.png} &

    %\imgRGB[100px 0px 0px 0px]{\figSeqVolume/ezgif-frame-001-render.jpeg} &
    %\imgRGB[45px 0px 0px 0px]{\figSeqBalloonw/training_ 0.png} &

    %\imgAtt[34px 0px 0px 0px]{\figSeqTwoDim/ezgif-frame-001-sal.png} &    
    \imgRGB[45px 0px 0px 0px]{\figSeqDynamicFace/15.png} &
    
    % \imgAtt[100px 0px 0px 0px]{\figSeqVolume/0_sal.png} 
    \imgRGB[45px 0px 0px 0px]{\figSeqJumping/23.png} &
    
    % \imgAtt[100px 0px 0px 0px]{\figSeqVolume/0_sal.png} 
    %\imgRGB[45px 0px 0px 0px]{\figSeqUmbrella/training_ 0.png} &
    \\


    \end{tabular}

    \vspace{-0.25cm}
    \caption{
        %\textbf{Post processing effect.} 
        Post processing helps remove small noisy regions from the raw results while maintaining thin features. 
    }
	
    \label{fig:postprocessed}
    \vspace{-0.25cm}
\end{figure}

}

==> fig/fig_pyramid/fig_pyramid.tex <==

{
\begin{figure*}[b]
    \centering
    \setlength{\tabcolsep}{1pt}
    
    % Set figure images paths for sequences
    % \newcommand{\figSeqJumping}{fig/fig_foreground/jumping}
    \newcommand{\figSeqBalloon}{fig/fig_pyramid/balloon}
    %\newcommand{\figSeqBalloonw}{fig/fig_anno/balloon2}
    \newcommand{\figSeqDynamicFace}{fig/fig_pyramid/dynamicFace}
    %\newcommand{\figSeqJumping}{fig/fig_post/jumping}
    %\newcommand{\figSeqSkating}{fig/fig_anno/skating}
    %\newcommand{\figSeqPlayground}{fig/fig_anno/playground}
    %\newcommand{\figSeqTruck}{fig/fig_anno/truck}
    \newcommand{\figSeqUmbrella}{fig/fig_pyramid/umbrella}

    % Set color remapping (can brighten images this way)
    \newcommand{\graymap}{{0 1}}
    \newcommand{\graymapBrighter}{{0.2 1.2}}
    \newcommand{\rgbcolormap}{{0 1 0 1 0 1}}
    \newcommand{\rgbcolormapFlip}{{0 1 0 1 0 1}}
    \newcommand{\rgbcolormapBrighter}{{1 0 1 0 1 0}}
    

    % Set image size
    \newcommand{\imgw}{0.19\linewidth} % 5-across figure
    \newcommand{\imgwhalf}{0.095\linewidth} % 5-across half-width figure
    %\newcommand{\imgh}{1in}
    
    % Command to draw an image with a different color map + crop as needed
    \newcommand{\imgRGB}[2][0px 0px 0px 0px]{\includegraphics[draft=\isdraft,width=\imgw,trim=#1,clip]{#2}}
    
    \newcommand{\imgAtt}[2][0px 0px 0px 0px]{\includegraphics[draft=\isdraft,decodearray={0.2 1.2},width=\imgw,trim=#1,clip]{#2}}

    \newcommand{\imgAttBr}[2][0px 0px 0px 0px]{\includegraphics[draft=\isdraft,decodearray={0.2 1.4},width=\imgw,trim=#1,clip]{#2}}

    % ^^^ NOTE DRAFT COMMAND!
    % Uncomment to actually show the pictures
    % ^^^

    \newcommand{\zoomRGB}[4]{
        \begin{tikzpicture}[
    		image/.style={inner sep=0pt, outer sep=0pt},
    		collabel/.style={above=9pt, anchor=north, inner ysep=0pt, align=center}, % scale=0.8
    		rowlabel/.style={left=9pt, rotate=90, anchor=north, inner ysep=0pt, scale=0.8, align=center},
    		subcaption/.style={inner xsep=0.75mm, inner ysep=0.75mm, below right},
    		arrow/.style={-{Latex[length=2.5mm,width=4mm]}, line width=2mm},
    		spy using outlines={rectangle, size=1.25cm, magnification=3, connect spies, ultra thick, every spy on node/.append style={thick}},
    		style1/.style={cyan!90!black,thick},
    		style2/.style={orange!90!black},
    		style3/.style={blue!90!black},
    		style4/.style={green!90!black},
    		style5/.style={white},
    		style6/.style={black},
        ]
        
        \node [image] (#1) {\imgRGB[100px 0px 0px 0px]{#2}};
        \spy[style5] on ($(#1.center)-#3$) in node (crop-#1) [anchor=#4] at (#1.#4);
        
        \end{tikzpicture}
    }

    \newcommand{\zoomAtt}[4]{
        \begin{tikzpicture}[
    		image/.style={inner sep=0pt, outer sep=0pt},
    		collabel/.style={above=9pt, anchor=north, inner ysep=0pt, align=center}, % scale=0.8
    		rowlabel/.style={left=9pt, rotate=90, anchor=north, inner ysep=0pt, scale=0.8, align=center},
    		subcaption/.style={inner xsep=0.75mm, inner ysep=0.75mm, below right},
    		arrow/.style={-{Latex[length=2.5mm,width=4mm]}, line width=2mm},
    		spy using outlines={rectangle, size=1.25cm, magnification=3, connect spies, ultra thick, every spy on node/.append style={thick}},
    		style1/.style={cyan!90!black,thick},
    		style2/.style={orange!90!black},
    		style3/.style={blue!90!black},
    		style4/.style={green!90!black},
    		style5/.style={white},
    		style6/.style={black},
        ]
        
        \node [image] (#1) {\imgAtt[100px 0px 0px 0px]{#2}};
        \spy[style5] on ($(#1.center)-#3$) in node (crop-#1) [anchor=#4] at (#1.#4);
        
        \end{tikzpicture}
    }

    \newcommand{\zoomAttBr}[4]{
        \begin{tikzpicture}[
    		image/.style={inner sep=0pt, outer sep=0pt},
    		collabel/.style={above=9pt, anchor=north, inner ysep=0pt, align=center}, % scale=0.8
    		rowlabel/.style={left=9pt, rotate=90, anchor=north, inner ysep=0pt, scale=0.8, align=center},
    		subcaption/.style={inner xsep=0.75mm, inner ysep=0.75mm, below right},
    		arrow/.style={-{Latex[length=2.5mm,width=4mm]}, line width=2mm},
    		spy using outlines={rectangle, size=1.25cm, magnification=3, connect spies, ultra thick, every spy on node/.append style={thick}},
    		style1/.style={cyan!90!black,thick},
    		style2/.style={orange!90!black},
    		style3/.style={blue!90!black},
    		style4/.style={green!90!black},
    		style5/.style={white},
    		style6/.style={black},
        ]
        
        \node [image] (#1) {\imgAttBr[100px 0px 0px 0px]{#2}};
        \spy[style5] on ($(#1.center)-#3$) in node (crop-#1) [anchor=#4] at (#1.#4);
        
        \end{tikzpicture}
    }

    \scriptsize
    \begin{tabular}{c c@{\hspace{0.2mm}} c@{\hspace{0.2mm}} c@{\hspace{0.2mm}} c@{\hspace{0.2mm}} c@{\hspace{0.2mm}} c}
    
    % Legend.
    % Note: first column is rotated sequence title
    
    & 
    Input & 
    w/o pyr & 
    Balanced $\lambdaSAFFsem$ + Global $\lambdaSAFFatt$ & 
    Weighted $\lambdaSAFFsem$ + Global $\lambdaSAFFatt$ & 
    Ours (Weighted $\lambdaSAFFsem$ + Weighted $\lambdaSAFFatt$) 
    \\

    %&
    %(a) Balloon NBoard &
    %(b) Umbrella
    %\\
    %%%%%%%%%%%%%%%%%%%%%%%%%
    % Sequence: Features

    % Labels
    %&
    %Balloon1-2 &
    %Balloon2-2 &
    %DynamicFace-2 & 
    %Jumping &
    %Umbrella
    %\\    

    \rotatebox{90}{\hspace{0.1cm} \seqBalloonNoticeBoard} &
     
    % \imgRGB[45px 0px 0px 0px]{\figSeqTwoDim/ezgif-frame-001.jpeg} &
    \imgRGB[45px 0px 0px 0px]{\figSeqBalloon/00006.png} &
    \imgRGB[45px 0px 0px 0px]{\figSeqBalloon/6.png} &
     \imgRGB[45px 0px 0px 0px]{\figSeqBalloon/6_0.png} &
     \imgRGB[45px 0px 0px 0px]{\figSeqBalloon/6_1.png} &
     \imgRGB[45px 0px 0px 0px]{\figSeqBalloon/6_ours.png} &

    %\imgRGB[100px 0px 0px 0px]{\figSeqVolume/ezgif-frame-001-render.jpeg} &
    %\imgRGB[45px 0px 0px 0px]{\figSeqBalloonw/00000.png} &

    %\imgAtt[34px 0px 0px 0px]{\figSeqTwoDim/ezgif-frame-001-sal.png} &    
    %\imgRGB[45px 0px 0px 0px]{\figSeqDynamicFace/00015.png} &
    
    % \imgAtt[100px 0px 0px 0px]{\figSeqVolume/0_sal.png} 
    %\imgRGB[45px 0px 0px 0px]{\figSeqJumping/00023.png} &
    
    % \imgAtt[100px 0px 0px 0px]{\figSeqVolume/0_sal.png} 
    %\imgRGB[45px 0px 0px 0px]{\figSeqUmbrella/00007.png} &
    \\


    % Images for pyramid preprocess
    %
    \rotatebox{90}{\hspace{0.4cm} \seqUmbrella} &
     
    % \imgRGB[45px 0px 0px 0px]{\figSeqTwoDim/ezgif-frame-001.jpeg} &
    \imgRGB[45px 0px 0px 0px]{\figSeqUmbrella/00019.png} &

    %\imgRGB[100px 0px 0px 0px]{\figSeqVolume/ezgif-frame-001-render.jpeg} &
    %\imgRGB[45px 0px 0px 0px]{\figSeqBalloonw/00000.png} &

    %\imgAtt[34px 0px 0px 0px]{\figSeqTwoDim/ezgif-frame-001-sal.png} &    
    %\imgRGB[45px 0px 0px 0px]{\figSeqDynamicFace/15_raw.png} &
    
    % \imgAtt[100px 0px 0px 0px]{\figSeqVolume/0_sal.png} 
    %\imgRGB[45px 0px 0px 0px]{\figSeqJumping/23_raw.png} &
    
    % \imgAtt[100px 0px 0px 0px]{\figSeqVolume/0_sal.png} 
    \imgRGB[45px 0px 0px 0px]{\figSeqUmbrella/19.png} &
    \imgRGB[45px 0px 0px 0px]{\figSeqUmbrella/19_0.png} &
    \imgRGB[45px 0px 0px 0px]{\figSeqUmbrella/19_1.png} &
    \imgRGB[45px 0px 0px 0px]{\figSeqUmbrella/19_ours.png} &
    
    \\
    
     %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    % Sequence: Pyramid preprocess
    
    % Labels for pyramid preprocess
    \rotatebox{90}{\hspace{0.2cm} \seqDynamicFace} &
     
    % \imgRGB[45px 0px 0px 0px]{\figSeqTwoDim/ezgif-frame-001.jpeg} &
    \imgRGB[45px 0px 0px 0px]{\figSeqDynamicFace/00004.png} &

    %\imgRGB[100px 0px 0px 0px]{\figSeqVolume/ezgif-frame-001-render.jpeg} &
    %\imgRGB[45px 0px 0px 0px]{\figSeqBalloonw/training_ 0.png} &

    %\imgAtt[34px 0px 0px 0px]{\figSeqTwoDim/ezgif-frame-001-sal.png} &    
    %\imgRGB[45px 0px 0px 0px]{\figSeqDynamicFace/15.png} &
    
    % \imgAtt[100px 0px 0px 0px]{\figSeqVolume/0_sal.png} 
    %\imgRGB[45px 0px 0px 0px]{\figSeqJumping/23.png} &
    
    % \imgAtt[100px 0px 0px 0px]{\figSeqVolume/0_sal.png} 
    
    \imgRGB[45px 0px 0px 0px]{\figSeqDynamicFace/4.png} &
    \imgRGB[45px 0px 0px 0px]{\figSeqDynamicFace/4_0.png} &
    \imgRGB[45px 0px 0px 0px]{\figSeqDynamicFace/4_1.png} &
    \imgRGB[45px 0px 0px 0px]{\figSeqDynamicFace/4_ours.png} &
    \\

    

    \end{tabular}

    \vspace{-0.25cm}
    \caption{
        \textbf{Pyramid construction varies final output quality after clustering.} Without the pyramid, key objects are missing or undersegmented. Our approach captures the objects with fewest errors compared to the variants.
        %Each approach uses our saliency-aware clustering \cref{alg:cluster}.
        \\
        Balanced $\lambdaSAFFsem$ + Global $\lambdaSAFFatt$: $\lambdaSAFFsem\! =\! \{\nicefrac{1}{3},\nicefrac{1}{3},\nicefrac{1}{3} \}$ with $\lambdaSAFFatt\! =\! \{1,0,0\}$
        \\
        Weighted $\lambdaSAFFsem$ + Global $\lambdaSAFFatt$: semantic attention pyramid
        %\cref{alg:pyr_final} 
        with $\lambdaSAFFatt\! =\! \{1,0,0\}$
        \\
        Ours (Weighted $\lambdaSAFFsem$ + Weighted $\lambdaSAFFatt$): Our semantic attention pyramid 
        %\cref{alg:pyr_final}.
    }
	
    \label{fig:pyramid_compare}
\end{figure*}
}


==> fig/fig_pyramiddiagram/fig_pyramiddiagram.tex <==
% Figma source:
% https://www.figma.com/file/7K2MNU1EsIEMZ1Or0IP5jK/CVPR-2023---Semantic-Attention-Flow-Fields?type=design&node-id=0-1&mode=design&t=BDgEcSafjDzIa1Ik-0

\begin{figure}[t]
    \includegraphics[width=\linewidth]{fig/fig_pyramiddiagram/pyramidconstruction.pdf}
    \caption{\textbf{Pyramid construction example.} This attempts to balance feature quality with computational cost by aggregating overlapping feature extraction blocks from different image resolutions.}
    \label{fig:pyramidconstruction}
\end{figure}

==> fig/fig_reb/dino_pillow.tex <==
{
\begin{figure}[t]
    \centering
    \setlength{\tabcolsep}{1pt}
    
    % Set figure images paths for sequences
    \newcommand{\figSeq}{fig/fig_limitations}
    \newcommand{\moviSeq}{fig/fig_limitations/movi_basket}

    % Set color remapping (can brighten images this way)
    \newcommand{\rgbcolormapBrighter}{{0.2 1.2 0.2 1.2 0.2 1.2}}
    \newcommand{\rgbcolormap}{{0 1 0 1 0 1}}

    % S et image size
    \newcommand{\imgw}{0.323\linewidth}
    \newcommand{\twoimgw}{0.5\linewidth}
    \newcommand{\tinyimgw}{0.2\linewidth}
    %\newcommand{\imgh}{1in}
    
    % Command to draw an image with a different color map + crop as needed
    \newcommand{\imgRGB}[2][0px 0px 0px 0px]{\includegraphics[draft=\isdraft,width=\imgw,trim=#1,clip]{#2}}
    
     \newcommand{\zoomRGB}[4]{
        \begin{tikzpicture}[
    		image/.style={inner sep=0pt, outer sep=0pt},
    		collabel/.style={above=9pt, anchor=north, inner ysep=0pt, align=center}, % scale=0.8
    		rowlabel/.style={left=9pt, rotate=90, anchor=north, inner ysep=0pt, scale=0.8, align=center},
    		subcaption/.style={inner xsep=0.75mm, inner ysep=0.75mm, below right},
    		arrow/.style={-{Latex[length=2.5mm,width=4mm]}, line width=2mm},
    		spy using outlines={rectangle, size=1cm, magnification=2, connect spies, ultra thick, every spy on node/.append style={thick}},
    		style1/.style={cyan!90!black,thick},
    		style2/.style={orange!90!black},
    		style3/.style={blue!90!black},
    		style4/.style={green!90!black},
    		style5/.style={white},
    		style6/.style={black},
        ]
        
        \node [image] (#1) {\imgRGB{#2}};
        \spy[style5] on ($(#1.center)-#3$) in node (crop-#1) [anchor=#4] at (#1.#4);
        
        \end{tikzpicture}
    }
    
    % ^^^ NOTE DRAFT COMMAND!
    % Uncomment to actually show the pictures
    % ^^^
    
    \vspace{-0.4cm}
    
    \begin{tabular}{c c c}
    
    % Legend.
    % Note: first column is rotated sequence title
  

    %%%%%%%%%%%%%%%%%%%%%%%%%
    % Sequence: Nvidia jumping sequence (non-instance)
    % &
    % \includegraphics[width=\imgw]{\figSeq/00001.png} &
    % \includegraphics[width=\imgw]{\figSeq/1_jump.png} &
    
    % \\[-1pt]

    (a) w. Post  &
    (b) w. Post + Oracle &
    (c) Feature Map
    \\
   

    %%%%%%%%%%%%%%%%%%%%%%%%%
    % Sequence: xxx

    % In general, we will pick a small set of sequences that show off key properties of our method.
    
    % \begin{tikzpicture}
    %     \node (saff-objects) { \includegraphics[width=\twoimgw]{\figSeq/6.png} };
    %     \node (input-rgb) [above right=-1.14cm and -1.92cm of saff-objects] { \includegraphics[width=\tinyimgw]{\figSeq/00006.png} };
    % \end{tikzpicture}
   
   %\includegraphics[width=\twoimgw]{\figSeq/00006.png} &
    \includegraphics[width=\imgw,trim=80px 0px 100px 0px,clip]{\figSeq/6_crf.png} &
    \includegraphics[width=\imgw,trim=80px 0px 100px 0px,clip]{\figSeq/6_oracle_pst.png} &
    
    
    %\includegraphics[width=\twoimgw]{\figSeq/test_gt.png}
    \includegraphics[width=\imgw,trim=80px 0px 100px 0px,clip]{\figSeq/test_gt.png} 
         

    \end{tabular}

    %\vspace{-0.5cm}
    %\caption{
    %    \YL{}
    %}
	
    \label{fig:dinopillow}
    \vspace{-0.2cm}
\end{figure}

}

==> fig/fig_reb/no_dep_rig.tex <==
{
\begin{figure}[t]
    \centering
    \setlength{\tabcolsep}{1pt}
    
    % Set figure images paths for sequences
    \newcommand{\figSeq}{fig/fig_limitations}
    \newcommand{\moviSeq}{fig/fig_limitations/movi_basket}

    % Set color remapping (can brighten images this way)
    \newcommand{\rgbcolormapBrighter}{{0.2 1.2 0.2 1.2 0.2 1.2}}
    \newcommand{\rgbcolormap}{{0 1 0 1 0 1}}

    % S et image size
    \newcommand{\imgw}{0.323\linewidth}
    \newcommand{\twoimgw}{0.5\linewidth}
    \newcommand{\tinyimgw}{0.2\linewidth}
    %\newcommand{\imgh}{1in}
    
    % Command to draw an image with a different color map + crop as needed
    \newcommand{\imgRGB}[2][210px 60px 150px 60px]{\includegraphics[draft=\isdraft,width=\imgw,trim=#1,clip]{#2}}
    
     \newcommand{\zoomRGB}[6]{
        \begin{tikzpicture}[
    		image/.style={inner sep=0pt, outer sep=0pt},
    		collabel/.style={above=9pt, anchor=north, inner ysep=0pt, align=center}, % scale=0.8
    		rowlabel/.style={left=9pt, rotate=90, anchor=north, inner ysep=0pt, scale=0.8, align=center},
    		subcaption/.style={inner xsep=0.75mm, inner ysep=0.75mm, below right},
    		arrow/.style={-{Latex[length=2.5mm,width=4mm]}, line width=2mm},
    		spy using outlines={rectangle, size=1cm, magnification=2, connect spies, ultra thick, every spy on node/.append style={thick}},
    		style1/.style={cyan!90!black,thick},
    		style2/.style={orange!90!black},
    		style3/.style={blue!90!black},
    		style4/.style={green!90!black},
    		style5/.style={white},
    		style6/.style={black},
        ]
        
        \node [image] (#1) {\imgRGB{#2}};
        \spy[style5] on ($(#1.center)-#3$) in node (crop-#1) [anchor=#4] at (#1.#4);
        \spy[style5] on ($(#1.center)-#5$) in node (crop-#1) [anchor=#6] at (#1.#6);
        
        \end{tikzpicture}
    }
    
    % ^^^ NOTE DRAFT COMMAND!
    % Uncomment to actually show the pictures
    % ^^^
    
    \vspace{-0.4cm}
    
    \begin{tabular}{c c c}
    
    % Legend.
    % Note: first column is rotated sequence title
  

    %%%%%%%%%%%%%%%%%%%%%%%%%
    % Sequence: Nvidia jumping sequence (non-instance)
    % &
    % \includegraphics[width=\imgw]{\figSeq/00001.png} &
    % \includegraphics[width=\imgw]{\figSeq/1_jump.png} &
    
    % \\[-1pt]

    
   

    %%%%%%%%%%%%%%%%%%%%%%%%%
    % Sequence: xxx

    % In general, we will pick a small set of sequences that show off key properties of our method.
    
    % \begin{tikzpicture}
    %     \node (saff-objects) { \includegraphics[width=\twoimgw]{\figSeq/6.png} };
    %     \node (input-rgb) [above right=-1.14cm and -1.92cm of saff-objects] { \includegraphics[width=\tinyimgw]{\figSeq/00006.png} };
    % \end{tikzpicture}
   
   %\includegraphics[width=\twoimgw]{\figSeq/00006.png} &
   
    \zoomRGB{ours}{\figSeq/57_rgb.png} {(0.4,-0.8)}{north east}{(-0.8,0.4)}{south west} &
    \zoomRGB{no-dep}{\figSeq/57_nodep.png} {(0.4,-0.8)}{north east}{(-0.8,0.4)}{south west}  &
    %\includegraphics[width=\imgw,trim=210px 60px 150px 60px,clip]{\figSeq/57_norig.png} 
    \zoomRGB{no-rig}{\figSeq/57_norig.png} {(0.4,-0.8)}{north east}{(-0.8,0.4)}{south west}
    
    %\includegraphics[width=\twoimgw]{\figSeq/test_gt.png}
         
    %(a) Ours  &
    %(b) w/o Depth &
    %(c) w/o Static
    

    \end{tabular}

    \vspace{-0.5cm}
    \caption{
        Left: ours, Middle: w/o Depth, Right: w/o Static
    }
	
    \label{fig:nondeprig}
    \vspace{-0.7cm}
\end{figure}

}

==> fig/fig_rgb/fig_rgb.tex <==
{
\begin{figure*}[t]
    \centering
    \setlength{\tabcolsep}{1pt}
    
    % Set figure images paths for sequences
    % \newcommand{\figSeqJumping}{fig/fig_foreground/jumping}
    \newcommand{\figSeqBalloon}{fig/fig_rgb/balloon}
    \newcommand{\figSeqBalloonw}{fig/fig_rgb/balloon2}
    \newcommand{\figSeqDynamicFace}{fig/fig_rgb/dynamicFace}
    \newcommand{\figSeqJumping}{fig/fig_rgb/jumping}
    \newcommand{\figSeqSkating}{fig/fig_rgb/skating}
    \newcommand{\figSeqPlayground}{fig/fig_rgb/playground}
    \newcommand{\figSeqTruck}{fig/fig_rgb/truck}
    \newcommand{\figSeqUmbrella}{fig/fig_rgb/umbrella}

    % Set color remapping (can brighten images this way)
    \newcommand{\graymap}{{0 1}}
    \newcommand{\graymapBrighter}{{0.2 1.2}}
    \newcommand{\rgbcolormap}{{0 1 0 1 0 1}}
    \newcommand{\rgbcolormapFlip}{{0 1 0 1 0 1}}
    \newcommand{\rgbcolormapBrighter}{{1 0 1 0 1 0}}
    

    % Set image size
    \newcommand{\imgw}{0.24\linewidth} % 5-across figure
    \newcommand{\imgwhalf}{0.12\linewidth} % 5-across half-width figure
    \newcommand{\imgh}{0.135\linewidth}
    
    % Command to draw an image with a different color map + crop as needed
    \newcommand{\imgRGB}[2][0px 0px 0px 0px]{\includegraphics[draft=\isdraft,width=\imgw,height=\imgh,trim=#1,clip]{#2}}
    
    \newcommand{\imgAtt}[2][0px 0px 0px 0px]{\includegraphics[draft=\isdraft,decodearray={0.2 1.2},width=\imgw,height=\imgh,trim=#1,clip]{#2}}

    \newcommand{\imgAttBr}[2][0px 0px 0px 0px]{\includegraphics[draft=\isdraft,decodearray={0.2 1.4},width=\imgw,height=\imgh,trim=#1,clip]{#2}}

    % ^^^ NOTE DRAFT COMMAND!
    % Uncomment to actually show the pictures
    % ^^^

    \newcommand{\zoomRGB}[4]{
        \begin{tikzpicture}[
    		image/.style={inner sep=0pt, outer sep=0pt},
    		collabel/.style={above=9pt, anchor=north, inner ysep=0pt, align=center}, % scale=0.8
    		rowlabel/.style={left=9pt, rotate=90, anchor=north, inner ysep=0pt, scale=0.8, align=center},
    		subcaption/.style={inner xsep=0.75mm, inner ysep=0.75mm, below right},
    		arrow/.style={-{Latex[length=2.5mm,width=4mm]}, line width=2mm},
    		spy using outlines={rectangle, size=1.25cm, magnification=3, connect spies, ultra thick, every spy on node/.append style={thick}},
    		style1/.style={cyan!90!black,thick},
    		style2/.style={orange!90!black},
    		style3/.style={blue!90!black},
    		style4/.style={green!90!black},
    		style5/.style={white},
    		style6/.style={black},
        ]
        
        \node [image] (#1) {\imgRGB[45px 0px 0px 0px]{#2}};
        \spy[style5] on ($(#1.center)-#3$) in node (crop-#1) [anchor=#4] at (#1.#4);
        
        \end{tikzpicture}
    }

    \newcommand{\zoomRGBDDNeRF}[4]{
        \begin{tikzpicture}[
    		image/.style={inner sep=0pt, outer sep=0pt},
    		collabel/.style={above=9pt, anchor=north, inner ysep=0pt, align=center}, % scale=0.8
    		rowlabel/.style={left=9pt, rotate=90, anchor=north, inner ysep=0pt, scale=0.8, align=center},
    		subcaption/.style={inner xsep=0.75mm, inner ysep=0.75mm, below right},
    		arrow/.style={-{Latex[length=2.5mm,width=4mm]}, line width=2mm},
    		spy using outlines={rectangle, size=1.25cm, magnification=3, connect spies, ultra thick, every spy on node/.append style={thick}},
    		style1/.style={cyan!90!black,thick},
    		style2/.style={orange!90!black},
    		style3/.style={blue!90!black},
    		style4/.style={green!90!black},
    		style5/.style={white},
    		style6/.style={black},
        ]
        
        \node [image] (#1) {\imgRGB[40px 0px 0px 0px]{#2}};
        \spy[style5] on ($(#1.center)-#3$) in node (crop-#1) [anchor=#4] at (#1.#4);
        
        \end{tikzpicture}
    }

    \newcommand{\zoomAtt}[4]{
        \begin{tikzpicture}[
    		image/.style={inner sep=0pt, outer sep=0pt},
    		collabel/.style={above=9pt, anchor=north, inner ysep=0pt, align=center}, % scale=0.8
    		rowlabel/.style={left=9pt, rotate=90, anchor=north, inner ysep=0pt, scale=0.8, align=center},
    		subcaption/.style={inner xsep=0.75mm, inner ysep=0.75mm, below right},
    		arrow/.style={-{Latex[length=2.5mm,width=4mm]}, line width=2mm},
    		spy using outlines={rectangle, size=1.25cm, magnification=3, connect spies, ultra thick, every spy on node/.append style={thick}},
    		style1/.style={cyan!90!black,thick},
    		style2/.style={orange!90!black},
    		style3/.style={blue!90!black},
    		style4/.style={green!90!black},
    		style5/.style={white},
    		style6/.style={black},
        ]
        
        \node [image] (#1) {\imgAtt[100px 0px 0px 0px]{#2}};
        \spy[style5] on ($(#1.center)-#3$) in node (crop-#1) [anchor=#4] at (#1.#4);
        
        \end{tikzpicture}
    }

    \newcommand{\zoomAttBr}[4]{
        \begin{tikzpicture}[
    		image/.style={inner sep=0pt, outer sep=0pt},
    		collabel/.style={above=9pt, anchor=north, inner ysep=0pt, align=center}, % scale=0.8
    		rowlabel/.style={left=9pt, rotate=90, anchor=north, inner ysep=0pt, scale=0.8, align=center},
    		subcaption/.style={inner xsep=0.75mm, inner ysep=0.75mm, below right},
    		arrow/.style={-{Latex[length=2.5mm,width=4mm]}, line width=2mm},
    		spy using outlines={rectangle, size=1.25cm, magnification=3, connect spies, ultra thick, every spy on node/.append style={thick}},
    		style1/.style={cyan!90!black,thick},
    		style2/.style={orange!90!black},
    		style3/.style={blue!90!black},
    		style4/.style={green!90!black},
    		style5/.style={white},
    		style6/.style={black},
        ]
        
        \node [image] (#1) {\imgAttBr[100px 0px 0px 0px]{#2}};
        \spy[style5] on ($(#1.center)-#3$) in node (crop-#1) [anchor=#4] at (#1.#4);
        
        \end{tikzpicture}
    }

    \scriptsize
    \begin{tabular}{c c@{\hspace{0.2mm}} c@{\hspace{0.2mm}} c@{\hspace{0.2mm}} c@{\hspace{0.2mm}}  c}
    
    % Legend.
    % Note: first column is rotated sequence title


     
    %%%%%%%%%%%%%%%%%%%%%%%%%
    % Sequence: Features

    % Labels
    &
    GT &
    NSFF~\cite{li2020neural} &
    \ddnerf~\cite{wu2022ddnerf} & 
    \titlename (ours) &
    \\    

    % %%%%%%%%%%%%%%%%%%%%%%%
    % % Sequence Notice Board
    % % Images for RGB 
    % %
    % \rotatebox{90}{\hspace{0.3cm} \seqBalloonNoticeBoard} &
     
    % \zoomRGB{balloonnb-gt}{\figSeqBalloon/cam01_2.png}{(-0.9,0.6)}{south west} &

    % \zoomRGB{balloonnb-nsff}{\figSeqBalloon/45_rgb_NSFF.png}{(-0.9,0.6)}{south west} &
    
    % \zoomRGBDDNeRF{balloonnb-ddnerf}{\figSeqBalloon/regular_rgb_000021.png}{(-0.7,0.6)}{south west} &
    
    % \zoomRGB{balloonnb-saff}{\figSeqBalloon/45_rgb.png}{(-0.9,0.6)}{south west}
    % \\
    
    % % Images for depth
    % %
    % &
    % &
    % \zoomRGB{balloonnb-depth-nsff}{\figSeqBalloon/45_depth_NSFF.png}{(-0.9,0.6)}{south west} &

    % \zoomRGB{balloonnb-depth-ddnerf}{\figSeqBalloon/45_depth_d2nerf.png}{(-0.9,0.6)}{south west} &

    % \zoomRGB{balloonnb-depth-saff}{\figSeqBalloon/45_depth_saff.png}{(-0.9,0.6)}{south west}
    % \\

    %%%%%%%%%%%%%%%%%%%%%
    % % Sequence Balloon Wall
    % %
    % \rotatebox{90}{\hspace{0.45cm} \seqBalloonWall} &
    
    % \imgRGB[45px 0px 0px 0px]{\figSeqBalloonw/cam01_3.png} &

    % \imgRGB[45px 0px 0px 0px]{\figSeqBalloonw/41_rgb_NSFF.png} &
    
    % \imgRGB[40px 0px 0px 0px]{\figSeqBalloonw/regular_rgb_017.png} &
    
    % \imgRGB[45px 0px 0px 0px]{\figSeqBalloonw/41_rgb.png}
    % \\  

    %%%%%%%%%%%%%%%%%%
    % Sequence Dynamic Face
    %
    \rotatebox{90}{\hspace{0.35cm} \seqDynamicFace} &

    \zoomRGB{dynamicface-gt}{\figSeqDynamicFace/cam09.png}{(0,-0.2)}{south west} &

    \zoomRGB{dynamicface-nsff}{\figSeqDynamicFace/56_rgb_NSFF.png}{(0,-0.2)}{south west} &
    
    \zoomRGBDDNeRF{dynamicface-ddnerf}{\figSeqDynamicFace/regular_rgb_020.png}{(0.2,-0.2)}{south west} &
    
    \zoomRGB{dynamicface-saff}{\figSeqDynamicFace/56_rgb.png}{(0,-0.2)}{south west}
    \\  
    
    % Images for depth
    %
    &
    &
    \zoomRGB{dynamicface-depth-nsff}{\figSeqDynamicFace/56_depth_NSFF.png}{(-0.2,0.1)}{south west} &

    \zoomRGB{dynamicface-depth-ddnerf}{\figSeqDynamicFace/regular_depth_020.png}{(0.45,0.18)}{south west} &

    \zoomRGB{dynamicface-depth-saff}{\figSeqDynamicFace/56_depth.png}{(-0.2,0.1)}{south west}
    \\
    
    %%%%%%%%%%%%%%%%%%%%
    %% Sequence Umbrella
    %% Images for RGB
    %% %
    % \rotatebox{90}{\hspace{0.7cm} \seqJumping} &
    
    % \imgRGB[45px 0px 0px 0px]{\figSeqJumping/cam07.png} &

    % \imgRGB[45px 0px 0px 0px]{\figSeqJumping/54_rgb_NSFF.png} &
    
    % \imgRGB[40px 0px 0px 0px]{\figSeqJumping/regular_rgb_018.png} &
    
    % \imgRGB[45px 0px 0px 0px]{\figSeqJumping/54_rgb.png}
    % \\ 

    %%%%%%%%%%%%%%%%%%%
    % Sequence skating
    % Images for RGB
    %
    \rotatebox{90}{\hspace{0.7cm} \seqSkating} &
    
    \zoomRGB{skating-gt}{\figSeqSkating/cam08.png}{(1.1,0.3)}{south east} &

    \zoomRGB{skating-nsff}{\figSeqSkating/55_rgb_NSFF.png}{(1.1,0.3)}{south east} &
    
    \zoomRGBDDNeRF{skating-ddnerf}{\figSeqSkating/regular_rgb_019.png}{(1.3,0.3)}{south east} &
    
    \zoomRGB{skating-saff}{\figSeqSkating/55_rgb.png}{(1.1,0.3)}{south east}
    \\  

    % Images for depth
    %
    &
    &
    \zoomRGB{dynamicface-depth-nsff}{\figSeqSkating/55_depth_NSFF.png}{(-0.9,0.6)}{south west} &

    \zoomRGB{dynamicface-depth-ddnerf}{\figSeqSkating/regular_depth_019.png}{(-0.9,0.6)}{south west} &

    \zoomRGB{dynamicface-depth-saff}{\figSeqSkating/55_depth.png}{(-0.9,0.6)}{south west}
    \\

    %%%%%%%%%%%%%%%%%%%
    % Sequence Umbrella
    % Images for RGB
    %
    \rotatebox{90}{\hspace{0.6cm} \seqUmbrella} &
     
    \zoomRGB{umbrella-gt}{\figSeqUmbrella/cam10.png}{(0.8,-0.33)}{south east} &

    \zoomRGB{umbrella-nsff}{\figSeqUmbrella/57_rgb_NSFF.png}{(0.75,-0.3)}{south east} &
    
    \zoomRGBDDNeRF{umbrella-ddnerf}{\figSeqUmbrella/regular_rgb_021.png}{(0.75,-0.3)}{south east} &
    
    \zoomRGB{umbrella-saff}{\figSeqUmbrella/57_rgb.png}{(0.75,-0.3)}{south east}
    \\  

    % Images for depth
    %
    &
    &
    \zoomRGB{umbrella-depth-nsff}{\figSeqUmbrella/57_depth_NSFF.png}{(-0.9,0.6)}{south west} &

    \zoomRGB{umbrella-depth-ddnerf}{\figSeqUmbrella/regular_depth_021.png}{(-0.9,0.6)}{south west} &

    \zoomRGB{umbrella-depth-saff}{\figSeqUmbrella/57_depth.png}{(-0.9,0.6)}{south west}

    \end{tabular}

    \vspace{-0.25cm}
    \caption{
        \textbf{\titlename does not degrade novel spacetime view synthesis or depth quality.} \ddnerf struggles on the NVIDIA Dynamic Scene Dataset sequences because of the large motions between cameras.
    }
	
    \label{fig:viewsynthesis_rgbdepth}
    \vspace{-0.25cm}
\end{figure*}

}

==> fig/fig_spacetime4Dclustering/fig_spacetime4Dclustering.tex <==
{
\begin{figure}[t]
    \centering
        
    \setlength{\tabcolsep}{1pt}
    
    % Set figure images paths for sequences
    % \newcommand{\figSeqJumping}{fig/fig_foreground/jumping}
    \newcommand{\figSeqBalloon}{fig/fig_spacetime4Dclustering/balloon}
    %\newcommand{\figSeqBalloonw}{fig/fig_anno/balloon2}
    %\newcommand{\figSeqDynamicFace}{fig/fig_anno/dynamicFace}
    \newcommand{\figSeqJumping}{fig/fig_spacetime4Dclustering/jumping}
    %\newcommand{\figSeqSkating}{fig/fig_anno/skating}
    %\newcommand{\figSeqPlayground}{fig/fig_anno/playground}
    \newcommand{\figSeqTruck}{fig/fig_spacetime4Dclustering/truck}
    %\newcommand{\figSeqUmbrella}{fig/fig_anno/umbrella}

    % Set color remapping (can brighten images this way)
    \newcommand{\graymap}{{0 1}}
    \newcommand{\graymapBrighter}{{0.2 1.2}}
    \newcommand{\rgbcolormap}{{0 1 0 1 0 1}}
    \newcommand{\rgbcolormapFlip}{{0 1 0 1 0 1}}
    \newcommand{\rgbcolormapBrighter}{{1 0 1 0 1 0}}
    

    % Set image size
    \newcommand{\imgw}{0.45\linewidth} % 5-across figure
    \newcommand{\imgwhalf}{0.225\linewidth} % 5-across half-width figure
    %\newcommand{\imgh}{1in}
    
    % Command to draw an image with a different color map + crop as needed
    \newcommand{\imgRGB}[2][0px 0px 0px 0px]{\includegraphics[draft=\isdraft,width=\imgw,trim=#1,clip]{#2}}
    
    \newcommand{\imgAtt}[2][0px 0px 0px 0px]{\includegraphics[draft=\isdraft,decodearray={0.2 1.2},width=\imgw,trim=#1,clip]{#2}}

    \newcommand{\imgAttBr}[2][0px 0px 0px 0px]{\includegraphics[draft=\isdraft,decodearray={0.2 1.4},width=\imgw,trim=#1,clip]{#2}}

    % ^^^ NOTE DRAFT COMMAND!
    % Uncomment to actually show the pictures
    % ^^^

    \newcommand{\zoomRGB}[4]{
        \begin{tikzpicture}[
    		image/.style={inner sep=0pt, outer sep=0pt},
    		collabel/.style={above=9pt, anchor=north, inner ysep=0pt, align=center}, % scale=0.8
    		rowlabel/.style={left=9pt, rotate=90, anchor=north, inner ysep=0pt, scale=0.8, align=center},
    		subcaption/.style={inner xsep=0.75mm, inner ysep=0.75mm, below right},
    		arrow/.style={-{Latex[length=2.5mm,width=4mm]}, line width=2mm},
    		spy using outlines={rectangle, size=1.25cm, magnification=3, connect spies, ultra thick, every spy on node/.append style={thick}},
    		style1/.style={cyan!90!black,thick},
    		style2/.style={orange!90!black},
    		style3/.style={blue!90!black},
    		style4/.style={green!90!black},
    		style5/.style={white},
    		style6/.style={black},
        ]
        
        \node [image] (#1) {\imgRGB[100px 0px 0px 0px]{#2}};
        \spy[style5] on ($(#1.center)-#3$) in node (crop-#1) [anchor=#4] at (#1.#4);
        
        \end{tikzpicture}
    }

    \newcommand{\zoomAtt}[4]{
        \begin{tikzpicture}[
    		image/.style={inner sep=0pt, outer sep=0pt},
    		collabel/.style={above=9pt, anchor=north, inner ysep=0pt, align=center}, % scale=0.8
    		rowlabel/.style={left=9pt, rotate=90, anchor=north, inner ysep=0pt, scale=0.8, align=center},
    		subcaption/.style={inner xsep=0.75mm, inner ysep=0.75mm, below right},
    		arrow/.style={-{Latex[length=2.5mm,width=4mm]}, line width=2mm},
    		spy using outlines={rectangle, size=1.25cm, magnification=3, connect spies, ultra thick, every spy on node/.append style={thick}},
    		style1/.style={cyan!90!black,thick},
    		style2/.style={orange!90!black},
    		style3/.style={blue!90!black},
    		style4/.style={green!90!black},
    		style5/.style={white},
    		style6/.style={black},
        ]
        
        \node [image] (#1) {\imgAtt[100px 0px 0px 0px]{#2}};
        \spy[style5] on ($(#1.center)-#3$) in node (crop-#1) [anchor=#4] at (#1.#4);
        
        \end{tikzpicture}
    }

    \newcommand{\zoomAttBr}[4]{
        \begin{tikzpicture}[
    		image/.style={inner sep=0pt, outer sep=0pt},
    		collabel/.style={above=9pt, anchor=north, inner ysep=0pt, align=center}, % scale=0.8
    		rowlabel/.style={left=9pt, rotate=90, anchor=north, inner ysep=0pt, scale=0.8, align=center},
    		subcaption/.style={inner xsep=0.75mm, inner ysep=0.75mm, below right},
    		arrow/.style={-{Latex[length=2.5mm,width=4mm]}, line width=2mm},
    		spy using outlines={rectangle, size=1.25cm, magnification=3, connect spies, ultra thick, every spy on node/.append style={thick}},
    		style1/.style={cyan!90!black,thick},
    		style2/.style={orange!90!black},
    		style3/.style={blue!90!black},
    		style4/.style={green!90!black},
    		style5/.style={white},
    		style6/.style={black},
        ]
        
        \node [image] (#1) {\imgAttBr[100px 0px 0px 0px]{#2}};
        \spy[style5] on ($(#1.center)-#3$) in node (crop-#1) [anchor=#4] at (#1.#4);
        
        \end{tikzpicture}
    }

    \scriptsize
    \begin{tabular}{c c@{\hspace{0.2mm}} c@{\hspace{0.2mm}}   c}
    
    % Legend.
    % Note: first column is rotated sequence title


    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
    % Labels
    &
    \seqJumping &
    \seqTruck
    \\    

    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    % Input images
    %
    \rotatebox{90}{\hspace{0.8cm} Input} &

    \imgRGB[45px 0px 0px 0px]{\figSeqJumping/00009.png} &
    
    \imgRGB[45px 0px 0px 0px]{\figSeqTruck/00017.png} 
    \\

    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    % 3D clustering
    
    % Labels for pyramid preprocess
    \rotatebox{90}{\hspace{0.35cm} w/ 3D} &

    \imgRGB[45px 0px 0px 0px]{\figSeqJumping/9_3D.png} &
    
    \imgRGB[45px 0px 0px 0px]{\figSeqTruck/17_3D.png} 
    \\

    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    % Spacetime clustering
    
    % Labels for pyramid preprocess
    \rotatebox{90}{\hspace{0.35cm} w/ spacetime} &

    \imgRGB[45px 0px 0px 0px]{\figSeqJumping/9_4D.png} &
    
    \imgRGB[45px 0px 0px 0px]{\figSeqTruck/17_4D.png} 
    \\

    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    % Projected 2D clustering
    \rotatebox{90}{\hspace{0.9cm} Ours} &

    \imgRGB[45px 0px 0px 0px]{\figSeqJumping/9.png} &
    
    \imgRGB[45px 0px 0px 0px]{\figSeqTruck/17.png} 
    \\


    \end{tabular}

    \vspace{-0.25cm}
    \caption{
        Clustering upon sampled 3D volume features or adding 4D spacetime features produces worse foregrounds qualitatively than just projected 2D feature clustering. This is because the narrow-baseline monocular input sometimes leads to noisy geometry estimation, and because the semantic edges must conform to the same geometry of the scene as the radiance. In 4D spacetime clustering, some clusters are confused or unnecessarily merged.
    }
	
    \label{fig:spacetime4dclustering}
\end{figure}

}

==> tab/tab_decay.tex <==
\begin{table}[t]
    \centering
    
    \caption{
        \textbf{Decaying semantic and attention information produces overall foregrounds.} While geometric alignment improves, semantic meaning also shifts, which harms the ability of the model to correctly identify salient objects. Metric: Adjusted Rand Index ($[-1,1]$, higher is better). 
        \label{tab:decay}
        }

    \vspace{-0.25cm}
    %\resizebox{\linewidth}{!}{
    \begin{tabular}{l r r r}
    
    \toprule
    {} & \datasplitInput & \datasplitCamZero & \datasplitTimeZero \\
    %{} & \multicolumn{3}{c}{ARI} \\
    
    \midrule
    
    \titlename (ours)           &  \textbf{0.653}   &  \textbf{0.634}   & \textbf{0.625}  \\
    \hspace{0.2cm} w/ decay     &  0.592            &  0.568            & 0.554  \\
    
    \bottomrule 
    
    \end{tabular}
    %}
\end{table}

==> tab/tab_necv.tex <==
\begin{table}[t]
    \centering
    
    \caption{
        \textbf{Dynamic scene decomposition.} \\
        % Dataset: \dataname. 
        Metric: Adjusted Rand Index ($[-1,1]$, higher is better). 
        \label{tab:scenedecomp}
        }

    \vspace{-0.25cm}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l r r r}
    
    \toprule
    {} & \datasplitInput & \datasplitCamZero & \datasplitTimeZero \\
    %{} & \multicolumn{3}{c}{ARI} \\
    \midrule 
    ProposeReduce (2D) &  \textbf{0.725} & \textbf{0.736}   & \textbf{0.742}  \\
    
    \semfeatnetwork (2D)                       &   0.501 & 0.495 & 0.321 \\
    \hspace{0.2cm} w/o pyr $\hat{\semfeat},\hat{\attfeat}$   &   0.470 & 0.464 & 0.346 \\
    
    \midrule
    \titlename (ours)                               &  \textbf{0.653}   &  \textbf{0.634}   & \textbf{0.625}  \\
    
    \bottomrule
    
    \end{tabular}
    }
    \vspace{-0.4cm}
\end{table}

==> tab/tab_pyramid.tex <==
\begin{table}[t]
    \centering
    
    \caption{
        \textbf{Pyramid weighting choice.} Even though in our final algorithm the coarse layer has smaller weight, it balances high resolution edges from fine layers and whole object features from coarse layers while reducing geometry conflicts, and mitigate the feature noise around edges.  \\
        % Dataset: \dataname. 
        Metric: Adjusted Rand Index ($[-1,1]$, higher is better). 
        \label{tab:pyramiddecompose}
        }

    \vspace{-0.25cm}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l r r r}
    
    \toprule
    {} & \datasplitInput & \datasplitCamZero & \datasplitTimeZero \\
    %{} & \multicolumn{3}{c}{ARI} \\
    
    \midrule
    SAFF  \\
    \hspace{0.2cm} w/o pyr $\hat{\semfeat},\hat{\attfeat}$  &  0.545            &  0.532            & 0.521  \\
    \midrule
    \titlename (ours)                               &  \textbf{0.653}   &  \textbf{0.634}   & \textbf{0.625}  \\
    \hspace{0.2cm} w/ pyr $\lambdaSAFFatt = \{1,0,0\}$    &  0.620            &  0.598            & 0.592  \\
    \hspace{0.2cm} w/ pyr $\lambdaSAFFatt = \{1,0,0\},$    &   \multirow{2}{*}{0.631}  & \multirow{2}{*}{0.612} & \multirow{2}{*}{0.601}\\
    \hspace{0.2cm}        $\lambdaSAFFsem\! =\! \{\nicefrac{1}{3},\nicefrac{1}{3},\nicefrac{1}{3} \}$ &     ~        &  ~   & ~ \\
    \bottomrule 
    
    \end{tabular}
    }
\end{table}

==> tab/tab_reb_1.tex <==
{

%\setlength{\tabcolsep}{0.25em}
\begin{table}[t]

    \vspace{-0.4cm}
    \centering
    
    \caption{
        Removing depth prior during training or static/dynamic. \\Metrics: L is LPIPS ($[0,1]$), S is SSIM ($[0,1]$), P is PSNR ($[0,\infty]$). \label{tab:reb_new_rgb}
    }
    \vspace{-0.25cm}
    
    \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{l c c c c c c c c c}
    \toprule
    {} & \multicolumn{3}{c}{\datasplitInput} & \multicolumn{3}{c}{\datasplitCamZero} & \multicolumn{3}{c}{\datasplitTimeZero} \\
    %{} & LPIPS & SSIM & PSNR & LPIPS & SSIM & PSNR & LPIPS & SSIM & PSNR \\
    {} & L \tridown & S \triup & P \triup & L & S & P & L & S & P \\
    \midrule
    %\ddnerf             & 0.115 & 0.790 & 23.91 & 0.228 & 0.565 & 18.04 & 0.344 & 0.309 & 13.85 \\
    NSFF (-masks)      &   0.070 & 0.805 & 23.92 &   0.100 & 0.762 & 21.68 &  0.302 & 0.386 & 14.92\\
    \hspace{0.2cm} w/o depth &  0.069 & 0.805 & 23.92 & 0.102 & 0.759 & 21.58 &  0.303 & 0.385 & 14.91\\
    \hspace{0.2cm} w/o static & 0.083 & 0.803 & 23.94 & 0.122 & 0.752 & 21.54 & 0.309 & 0.390 & 14.96\\
    \titlename (ours)   &   0.070 & 0.805 & 23.92 &   0.100 & 0.762 & 21.70 &  0.302 & 0.386 & 14.93 \\
    \hspace{0.2cm} w/o depth   & 0.070  & 0.805 & 23.92 & 0.103  & 0.760 & 21.55 & 0.303  & 0.386 & 14.91\\
    \hspace{0.2cm} w/o static   & 0.089 & 0.801 & 23.84 &  0.128 & 0.751 & 21.50 &  0.311 & 0.391 & 14.96\\
    
    \bottomrule
    
    \end{tabular}
    }
    \vspace{-0.4cm}
    
\end{table}
}

==> tab/tab_reb_2.tex <==
{


\begin{table}[ht]

\vspace{-0.4cm}
\newcommand{\yes}{\ding{51}}
    \newcommand{\no}{\ding{53}}
    \newcommand{\notapplicable}{N/A}
    \newcommand{\figSeq}{fig/fig_limitations}
    \newcommand{\moviSeq}{fig/fig_limitations/movi_basket}

    % Set color remapping (can brighten images this way)
    \newcommand{\rgbcolormapBrighter}{{0.2 1.2 0.2 1.2 0.2 1.2}}
    \newcommand{\rgbcolormap}{{0 1 0 1 0 1}}

    % S et image size
    \newcommand{\imgw}{0.2\linewidth}
    \newcommand{\twoimgw}{0.5\linewidth}
    \newcommand{\tinyimgw}{0.2\linewidth}
\begin{minipage}[tb]{0.6\linewidth}
\centering
\resizebox{0.8\linewidth}{!}{
\begin{tabular}{ l  r  r }
    \toprule
    %{} & \multirowcell{2}{Dynamic\\(video)} &
    %\multirowcell{2}{Mono-\\cular} &
    %\multirowcell{2}{Real\\world} & \multirowcell{2}{3D} & 
    %\multirowcell{2}{No seg.\\clue} &
    %\multirowcell{2}{Learning} & 
    %\multirowcell{2}{Adaptive \\ \# objects} &
    %\multirowcell{2}{Object-\\level}\\
    %\\
    
    ~ & Ours & Oracle\\
    \midrule
    Input & 0.653 & 0.834 \\
    Fix Cam 0 & 0.634 & 0.806 \\
    Fix Time 0 & 0.625 & 0.800 \\
    \bottomrule

   \end{tabular}}
   \vspace{-0.3cm}
    \caption{\triup Adjusted Rand Index ($[-1,1]$)}
    %\label{table:student}
\end{minipage}\hfill
\begin{minipage}[tb]{0.4\linewidth}
\centering
\includegraphics[width=0.9\linewidth, trim=80px 0px 100px 0px, clip]{\figSeq/test_gt.png}
%\vspace{-0.25cm}
%\captionof{figure}{Feature Map}
%\label{fig:image}
\end{minipage}
\vspace{-0.5cm}
\end{table}



}

==> tab/tab_reb_3.tex <==

\begin{table}[t]

\vspace{0.3cm}
    \centering
    \setlength{\tabcolsep}{1.25em}
    \caption{
        %ProposeReduce pretrained on DAVIS-UVOS. %~\cite{Caelles_arXiv_2019}
        % Dataset: \dataname. 
        Metric: \triup IoU/Jaccard index ($[0,1]$).
        \label{tab:reb_foregroundsegmentation}
    }

    \vspace{-0.25cm}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l r r r}
    
    \toprule
    {} & \datasplitInput & \datasplitCamZero & \datasplitTimeZero \\
    \midrule
    ProposeReduce (UVOS)          &  0.609 & 0.464   & 0.591  \\
    %DINO-ViT (2D)  &  0.381 & 0.382  & 0.357  \\
    %\midrule
    %NSFF --- blend $v$          & 0.322 & 0.309 & 0.268 \\
    %\ddnerf --- blend $v$       &  0.470 & 0.334 & 0.269 \\ 

    \titlename     &  0.609  &  0.589  & 0.572  \\
    %\hspace{0.2cm} w/o depth    &  ~ & ~ & ~ \\
    %\hspace{0.2cm} w/o static    &  ~ & ~ & ~ \\
    \hspace{0.2cm} w/ post process    &  0.720 & 0.694  & 0.679 \\
    \bottomrule
    \vspace{-0.5cm}
    \end{tabular}
    }
    
    \vspace{-0.5cm}
\end{table}

==> tab/tab_related.tex <==
{

\begin{table*}[t]
    \centering

    \newcommand{\yes}{\ding{51}}
    \newcommand{\no}{\ding{53}}
    \newcommand{\notapplicable}{N/A}

\adjustbox{valign=t}{
\begin{minipage}[t]{0.66\linewidth}
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l c c c  c c c c c }
    
    \toprule
    {} & \multirowcell{2}{Dynamic\\(video)} &
    \multirowcell{2}{Mono-\\cular} &
    \multirowcell{2}{Real\\world} & \multirowcell{2}{3D} & 
    \multirowcell{2}{No seg.\\clue} &
    \multirowcell{2}{Learning} & 
    \multirowcell{2}{Adaptive \\ \# objects} &
    \multirowcell{2}{Object-\\level}\\
    \\
    \midrule
    
    %IODINE\cite{greff2019multiobject} & \no & \yes & \no & \no & \yes & \no & \no & \yes\\
    %MONET\cite{burgess2019monet} & \no & \yes & \no & \no & \yes & \no & \no & \yes\\
    %Slot Attention\cite{locatello2020object} & \no & \yes & \no & \no & Mask & Large-scale & \no & \yes\\
    
    %\midrule
    
    %SIMONe\cite{Kabra2021SIMONeVT} & \yes & \yes & \no & \no & \yes & \no & \no & \yes\\
    %SAVi\cite{kipf2022conditional} & \yes & \yes & \no & \no & Mask & Large-scale & \no & \yes\\

    ProposeReduce\cite{lin2021video} & \yes & \yes & \yes & \no & \yes & T & \yes & \yes\\
    SAVi++\cite{elsayed2022savipp} & \yes & \yes & \yes & \no & Mask & T & \no & \yes\\
    
    \midrule
    
    ObSuRF\cite{stelzner2021decomposing} & \no & \no & \no & \yes & \yes & \no & \no & \yes\\
    uORF\cite{yu2022unsupervised}& \no & \no & \no & \yes & \yes & \no & \no & \yes\\
    %COLF\cite{smith2022colf} & \no & \no & \no & \yes & \yes & \no & \no & \yes\\
    
    %\midrule
    % PNF\cite{Kundu_2022_CVPR} & \yes & \yes & \yes & \yes & Mask & \no & \no & \yes \\
    %Panoptic-NeRF \cite{fu2022panoptic} & \yes & \yes & \yes & \no\\
    % Object-NeRF \cite{yang2021objectnerf} & \no & \no & \yes & \yes & Mask & \no & \no & \yes\\
    
    \midrule
    DFF\cite{kobayashi2022distilledfeaturefields} & \no & \no & \yes & \yes & User & P & \yes & \yes\\
    N3F\cite{tschernezki22neural} & \yes & \yes & \yes & \yes & User & P & \yes & \yes\\
    
    \midrule
    NSFF\cite{li2020neural} & \yes & \yes & \yes & \yes & Mask & \no & \notapplicable & \notapplicable \\
    D$^2$NeRF\cite{wu2022ddnerf} & \yes & \yes & \yes & \yes & \yes & \no & \notapplicable & \notapplicable \\
    \midrule
    \titlename (this paper) & \yes & \yes & \yes & \yes & \yes & P & \yes & \yes\\
    
    \bottomrule
    \end{tabular}
    }
\end{minipage}
}
%
\quad
%
\adjustbox{valign=t}{
\begin{minipage}[t]{0.29\linewidth}
    \caption{
        Comparing related work in segmentation and scene decomposition shows the unstudied area of dynamic 3D segmentation without explicit segmentation clues. We investigate whether saliency provides similar clues for monocular video. 
        % Supplemental material has an expanded table.\\
        Learning: Large-scale training data:\\
        T: Supervised task-specific data.\\
        P: Generic features (e.g., ImageNet).\\
        \no: No features used.
        \label{tab:relatedwork}
    }
\end{minipage}
}
\vspace{-0.7cm}
\end{table*}

}

==> tab/tab_related_expanded_supplemental_hack.tex <==
{
\begin{table*}[b]
    \centering

    \newcommand{\yes}{\ding{51}}
    \newcommand{\no}{\ding{53}}
    \newcommand{\notapplicable}{N/A}
    
    \caption{
        An comparison of related work in scene decomposition shows the unstudied area of real-world dynamic 3D segmentation without explicit segmentation clues. We investigate whether saliency can provide similar clues for the monocular video case. From this table, the closest related method is N3F; however, they take user input to define their segmentation.
       \\
        Learning: Large-scale training data:\\
        T: Supervised task-specific data.\\
        P: Generic features (e.g., ImageNet).\\
        \no: No features used.
        \label{tab:relatedwork_expanded}
    }
    %\resizebox{\linewidth}{!}{
    \begin{tabular}{l c c c  c c c c c }
    
    \toprule
    {} & \multirowcell{2}{Dynamic\\(video)} &
    \multirowcell{2}{Monocular} &
    \multirowcell{2}{Real\\world} & \multirowcell{2}{3D} & \multirowcell{2}{No seg. \\clue} &
    \multirowcell{2}{Learning} & 
    \multirowcell{2}{Adaptive \\ \# objects} &
    \multirowcell{2}{Object-\\level}\\
    \\
    \midrule
    
    IODINE\cite{greff2019multiobject} & \no & \yes & \no & \no & \yes & \no & \no & \yes\\
    MONET\cite{burgess2019monet} & \no & \yes & \no & \no & \yes & \no & \no & \yes\\
    Slot Attention\cite{locatello2020object} & \no & \yes & \no & \no & Mask & T & \no & \yes\\
    
    \midrule
    
    SIMONe\cite{Kabra2021SIMONeVT} & \yes & \yes & \no & \no & \yes & \no & \no & \yes\\
    SAVi\cite{kipf2022conditional} & \yes & \yes & \no & \no & Mask & T & \no & \yes\\
    SAVi++\cite{elsayed2022savipp} & \yes & \yes & \yes & \no & Mask & T & \no & \yes\\
    
    \midrule
    
    ObSuRF\cite{stelzner2021decomposing} & \no & \no & \no & \yes & \yes & \no & \no & \yes\\
    uORF\cite{yu2022unsupervised}& \no & \no & \no & \yes & \yes & \no & \no & \yes\\
    COLF\cite{smith2022colf} & \no & \no & \no & \yes & \yes & \no & \no & \yes\\
    
    \midrule
    
    PNF\cite{Kundu_2022_CVPR} & \yes & \yes & \yes & \yes & Mask & \no & \no & \yes \\
    %Panoptic-NeRF \cite{fu2022panoptic} & \yes & \yes & \yes & \no\\
    Object-NeRF \cite{yang2021objectnerf} & \no & \no & \yes & \yes & Mask & \no & \no & \yes\\
    
    \midrule
    DFF\cite{kobayashi2022distilledfeaturefields} & \no & \no & \yes & \yes & User & P & \yes & \yes\\
    N3F\cite{tschernezki22neural} & \yes & \yes & \yes & \yes & User & P & \yes & \yes\\
    
    \midrule
    ProposeReduce\cite{lin2021video} & \yes & \yes & \yes & \no & \yes & T & \yes & \yes\\
    NSFF\cite{li2020neural} & \yes & \yes & \yes & \yes & Mask & \no & \notapplicable & \notapplicable\\
    D$^2$NeRF\cite{wu2022ddnerf} & \yes & \yes & \yes & \yes & \yes & \no & \notapplicable & \notapplicable\\
    \midrule
    \titlename (this paper) & \yes & \yes & \yes & \yes & \yes & P & \yes & \yes\\
    
    \bottomrule
    
    \end{tabular}
    %}
\end{table*}
}

==> tab/tab_rgb_noharm.tex <==
{
\setlength{\tabcolsep}{0.25em}
\begin{table}[tb]

    \centering
    
    \caption{
        \textbf{SAFF does not degrade image quality.} Adding semantics and attention on the same backbone produces the same image quality as NSFF~\cite{li2020neural}. Metrics: L is LPIPS ($[0,1]$, lower is better), S is SSIM ($[0,1]$, higher is better), P is PSNR ($[0,\infty]$, higher is better). \label{tab:rgb_noharm}
    }
    %\vspace{-0.25cm}
    
    \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{l c c c c c c c c c}
    \toprule
    {} & \multicolumn{3}{c}{\datasplitInput} & \multicolumn{3}{c}{\datasplitCamZero} & \multicolumn{3}{c}{\datasplitTimeZero} \\
    %{} & LPIPS & SSIM & PSNR & LPIPS & SSIM & PSNR & LPIPS & SSIM & PSNR \\
    {} & L \tridown & S \triup & P \triup & L & S & P & L & S & P \\
    \midrule
    \ddnerf             & 0.115 & 0.790 & 23.91 & 0.228 & 0.565 & 18.04 & 0.344 & 0.309 & 13.85 \\
    NSFF w/o masks      & 0.070 & 0.805 & 23.92 &   0.100 & 0.762 & 21.68 &  0.302 & 0.386 & 14.92 \\
    \titlename (ours)   & 0.070 & 0.805 & 23.92 &   0.100 & 0.762 & 21.70 &  0.302 & 0.386 & 14.93 \\
    \bottomrule
    
    \end{tabular}
    }
    %\vspace{-0.5cm}
    
\end{table}
}

==> tab/tab_spacetime4Dclustering.tex <==
\begin{table}[t]
    \centering
    
    \caption{
        \textbf{3D volume clustering produces worse 2D segmentations than projected 2D clustering.} This is because precise localization of 3D geometry is difficult from monocular inputs for dynamic scenes. 4D spacetime clustering also produces worse foregrounds. Metric: Adjusted Rand Index ($[-1,1]$, higher is better). 
        \label{tab:spacetime4dclustering}
    }

    \vspace{-0.25cm}
    %\resizebox{\linewidth}{!}{
    \begin{tabular}{l r r r}
    
    \toprule
    {} & \datasplitInput & \datasplitCamZero & \datasplitTimeZero \\
    %{} & \multicolumn{3}{c}{ARI} \\
    
    \midrule
    
    \titlename (ours)                               &  \textbf{0.653}   &  \textbf{0.634}   & \textbf{0.625}  \\
    \hspace{0.2cm} in 3D                            &  0.594   &  0.578 &
    0.566 \\
    \hspace{0.2cm} in 4D spacetime                  &  0.482            &  0.464            & 0.452  \\
    
    \bottomrule 
    
    \end{tabular}
    %}
\end{table}

==> tex/02_related_long.tex <==
% Forward declaration of related work
\vspace{-0.25cm} % Make sure it's on the previous page...
\input{tab/tab_related}

\section{Related Work}
\label{sec:relatedwork}

%\jt{To add still: \href{https://arxiv.org/pdf/2209.14860.pdf}{https://arxiv.org/pdf/2209.14860.pdf}, \href{https://github.com/Alxead/SFC}{https://github.com/Alxead/SFC}}

The task of decomposing a scene into regions of interest is long studied in computer vision, including work in class, instance, and panoptic segmentation in high-level or top-down vision, and in work using low-level or bottom-up cues like motion. We focus on lower-level related works, with recent progress on images (IODINE~\cite{greff2019multiobject}, MONET~\cite{burgess2019monet}, Slot Attention~\cite{locatello2020object}) and on videos (SIMONe~\cite{Kabra2021SIMONeVT}, SAVi~\cite{kipf2022conditional}). 
Research has also investigated decomposition into layers (deformable sprites~\cite{ye2022sprites}, DTI-Sprites~\cite{Monnier_2021_ICCV}) and via in-the-wild databases using deep generative models (GIRAFFE~\cite{Niemeyer2020GIRAFFE}). 
One recent example, SAVi++\cite{elsayed2022savipp}, uses slot attention to define objects in 2D real-world videos. Stable performance is achieved when providing a segmentation mask for the first frame, with validation on the driving Waymo Open Dataset~\cite{Sun_2020_CVPR}. Our work attempts 3D scene decomposition for a casual monocular video without being given any scene masks (Tab.~\ref{tab:relatedwork}).

\vspace{-0.1cm}
\paragraph{Scene Decomposition with NeRFs}
\label{sec:relatedwork_withnerfs}

Neural Radiance Fields (NeRF)~\cite{10.1111:cgf.14505} have spurred new scene decomposition research through volume optimization.
ObSuRF~\cite{stelzner2021decomposing} and uORF~\cite{yu2022unsupervised} are unsupervised slot attention works that bind a latent code to each object. 
Unsupervised decomposition is also explored for light fields in COLF~\cite{smith2022colf}. 
For dynamic scenes, some works like NeuralDiff~\cite{tschernezki21neuraldiff} and \ddnerf~\cite{wu2022ddnerf} focus on foreground separation, where foreground is defined to contain moving objects. 
Other works like N3F~\cite{tschernezki22neural} and occlusions-4d~\cite{vanhoorick2022revealing} also decompose foregrounds into individual objects. 
N3F requires user input to specify which object to segment, and occlusions-4d takes RGB point clouds as input. 
Our work belongs to this category, and attempts to recover a segmented dynamic scene from a monocular RGB video without added markup or masks.

\vspace{-0.1cm}
\paragraph{Neural Fields Beyond Radiance}
\label{sec:relatedwork_beyondradiance}

Research has begun to add non-color information to neural volumes to aid decomposition via additional feature heads on the MLP. 
% As NeRF has achieved success in both geometry and appearance reconstruction by only using 2D color images use pose as supervision, people found that adding more heads parallel to appearance head and geometry head can help distill other information into the underlying neural fields with additional 2D supervision. 
For instance, iLabel~\cite{Zhi:etal:ICCV2021} adds a semantic head to propagate user-provided segmentations in the volume. PNF~\cite{Kundu_2022_CVPR} and Panoptic-NeRF~\cite{fu2022panoptic} attempt panoptic segmentation within neural fields, and Object-NeRF integrates instance segmentation masks into the field during optimization~\cite{yang2021objectnerf}. 
Research also investigates how to apply large pre-trained features to neural fields, such as \semfeatnetwork.

\vspace{-0.1cm}
\paragraph{\semfeatnetwork for Semantics and Saliency}
% \semfeatnetwork = DINO-ViT
\semfeatnetwork is a self-supervised transformer architecture introduced by Caron et al.~\cite{caron2021emerging}. After pretraining on a large dataset, \semfeatnetwork can extract generic semantic information from an image input. Amir et al.~\cite{amir2021deep} shows that \semfeatnetwork features with $k$-means clustering can achieve co-segmentation across a video. Seitzer et al.~\cite{seitzer2022bridging} combine slot attention and \semfeatnetwork features for object-centric learning on real-world 2D data. TokenCut~\cite{wang2022tokencut} combines \semfeatnetwork with normalized cut to perform foreground segmentation on natural images. Deep Spectral Segmentation~\cite{melaskyriazi2022deep} show that graph Laplacian processing of \semfeatnetwork features provides unsupervised foreground segmentation, and Selfmask~ \cite{shin2022selfmask} show that these features can provide object saliency masks. %Tumanyan et al.~\cite{Tumanyan2022} transfer \semfeatnetwork features for creative appearance changes. 
Our approach considers the \semfeatnetwork clustering and saliency findings for the setting of 3D decomposition from monocular video.

\vspace{-0.1cm}
\paragraph{\semfeatnetwork Fields}
\label{sec:concurrent}

Concurrent works have integrated \semfeatnetwork features into neural fields. DFF~\cite{kobayashi2022distilledfeaturefields} distills features for dense multi-view static scenes with user input for segmentation, while we target casual monocular videos and explore saliency for segmentation. 
% Their segmentation also only happens when there is user input. 
N3F~\cite{tschernezki22neural} expands NeuralDiff to dynamic scenes, and relies on user input for segmentation. AutoLabel~\cite{blomqvist2022baking} uses \semfeatnetwork features to accelerate segmentation in static scenes given a ground truth segmentation mask.
%; we show that segmentation is possible with DINO-ViT alone. 
%
Other works use \semfeatnetwork differently. FeatureRealisticFusion~\cite{Mazur:etal:ARXIV2022} use \semfeatnetwork in an online feature fusion task, focusing on propagating user input, and 
%Instead of training under the DINO-ViT results on groundtruth images, 
NeRF-SOS~\cite{Fan2022} use 2D DINO-ViT to process NeRF-rendered multi-view RGB images of a static scene.
% they also perform clustering on resulting feature field, but their object masks are binary.
%
In contrast to these works, we consider real-world casual monocular videos, recover and semantically-decompose a 3D scene, then explore whether saliency can avoid the need for masks or user input in segmenting objects.

% Forward declaration of overview pipeline figure
% 
\input{fig/fig_overview/fig_overview.tex}

==> tex/03a_methods_nsff_long.tex <==
\subsection{Initial Dynamic Neural Volume Representation}
\label{sec:method_basic}

Following NSFF, our initial representation comprises a static NeRF $\network^\static$ and a dynamic NeRF $\network^\dynamic$. %\EL{Is it okay to use theta to represent the parameters for both?}
%\jt{Good catch, but I think we should let this one slip. We can assume the superscript is sufficient.}
For each timestep $\timestep$, we query each network with a 3D field position $\xpos$ and a ray direction $\direction$. The static network predicts a color $\xcol$, density $\sigma$, and blending weight $v$ (\cref{eq:nsff_static}), and the dynamic network predicts time-varying color $\xcol_i$, density $\sigma_i$, scene flow $\flowscene_i$, and occlusion weights $w_i$ (\cref{eq:nsff_dynamic}). In both network architectures, $\direction$ is added to a late separate head and only conditions the estimation of color $\xcol$.
%
\begin{align}
\label{eq:nsff_static}
    % (c, \sigma, v) = F_\Theta^{st}(x, d) \\
    \network^\static : (\xpos, \direction) \hspace{0.3cm} &\rightarrow (\xcol^\static, \sigma^\static, v) \\
\label{eq:nsff_dynamic}
    % (c_i, \sigma_i, F_i, W_i) = F_\Theta^{dy}(x, d, i) \\
    \network^\dynamic : (\xpos, \direction, \timestep) &\rightarrow (\xcol_i^\dynamic, \sigma_i^\dynamic, \flowscene_i, w_i)
\end{align}

To produce a pixel's color, we sample points at distances $t$ along the ray $\xpos_t=\xpos-\direction t$ between near and far planes $t_n$ to $t_f$, query each network $\network^\static(\xpos_t,\direction)$, then integrate transmittance $T$, density $\sigma$, and color along the ray from these samples~\cite{mildenhall2020nerf}.
%Start from the nearest sample ($t_n$), the transmittance $T$ of the pixel ray is calculated while traversing all points along the ray towards $t_f$. 
For brevity, we omit evaluating at $\xpos_t,\direction$, \eg, $\sigma^\static(\xpos_t)$ is simply $\sigma^\static$; $\xcol^\static(\xpos_t,\direction)$ is simply $\xcol^\static$.

%For each sample point, we start by blending the static and dynamic densities into a combined density: \YL{This is wrong; they first time sigma and color, then weighted combining}
%
\begin{align}
\label{eq:nsff_density_staticdynamic_sum}
    % \sigma_i^\combined(\xpos_t) = v(\xpos_t)\sigma^\static(\xpos_t) + (1-v(\xpos_t))\sigma_i^\dynamic(\xpos_t)
    \sigma_i = v\sigma^\static + (1-v)\sigma_i^\dynamic
\end{align}

%One core problem with blended static and dynamic formulations is how to encourage the dynamic network not to represent static or view-dependent content, as the video could entirely be explained by the dynamic network. \jt{The NSFF code deploys an additional mask loss from supervised hand-drawn segmentations to improve dynamic object quality. We will show that integrating semantic and attention fields can improve upon this difficult segmentation task without requiring any hand-drawn dynamic object masks.}
%\YL{Don't think we have enough results to support this; should remove this paragraph}
% Note that the static network's density prediction does not take time step $i$ as input, and the weight prediction $v(t)$ comes from static network.  

We produce a combined color from the static and dynamic colors by multiplication with their densities:
%
\begin{align}
\label{eq:nsff_color_staticdynamic_sum}
    % \sigma_i^\combined(\xpos_t)c_i^\combined(\xpos_t) = v(\xpos_t)c^\static(\xpos_t)\sigma^\static(\xpos_t) + (1-v(\xpos_t))c_i^\dynamic(\xpos_t)\sigma_i^\dynamic(\xpos_t)
    \sigma_i \xcol_i = v\sigma^\static\xcol^\static + (1-v)\sigma_i^\dynamic\xcol_i^\dynamic
\end{align}

%Transmittance integrates density up to the current sampled point under Beer-Lambert volume attenuation:
% % Intuitively, as the ray departs from the nearest sample $t_f$, the transmittance keeps decreasing as more non-empty samples are met, implying that the later samples are less likely to be seen at the camera pixel.
% %
% \begin{align}
% \label{eq:nsff_transmittance}
%     T_i = \exp\left( - \int_{t_n}^{t} \sigma_i \, dt\right)
% \end{align}

%The final color to be rendered for this ray $r_i$ would be the integral of the weighted color values alongside the ray from $t_n$ to $t_f$ by \ref{color integral}. The weight for each point $t$ would be transmittance $T_i^{cb}(t)$ times density $\sigma_i^{cb}(t)$, so that only points that are not occluded and are non-empty would dominate the pixel color. As there are infinite points along the ray, approximate the integral by performing the summation over all queried point samples, each $t \in [t_n, t_f]$.
Given that transmittance integrates density up to the current sampled point under Beer-Lambert volume attenuation, the rendered pixel color for the ray is computed as:
%
\begin{align}
\label{eq:nsff_colorintegral}
    % \hat{\xcol}_i^\combined(\ray_i) =  \int_{t_n}^{t_f} {T_i^\combined(\xpos_t)\sigma_i^\combined(\xpos_t)c_i^\combined(\xpos_t) \, dt}
    \pixcol_i =  \int_{t_n}^{t_f} {T_i \sigma_i \xcol_i \, dt} \hspace{0.2cm}\text{where}\hspace{0.2cm} T_i = \exp\left( - \int_{t_n}^{t} \sigma_i \, dt\right)
\end{align}

To encourage the optimization to reconstruct all input images, for each ray $\ray_i$, we compute a photometric loss $L_{\hat{\xcol}}$ as the MSE between the rendered color and the input color: 
%
\begin{align}
\label{eq:nsff_loss_color}
    \lossNSFFPixCol = \frac{1}{|\mathcal{R}|} \sum\limits_{\ray_i \in \mathcal{R}}||\pixcol_i(\ray_i) - \pixcol_i^\dagger(\ray_i)||_2^2
\end{align}

\paragraph{Scene Flow} Defining correspondence over time is important for monocular input as it lets us penalize a reprojection error with neighboring frames $j \in \mathcal{N}(i)$, e.g., where $j=i+1$ or $j=i-1$. We use notation $_{i\rightarrow{j}}$ for the projection of frame $i$ onto frame $j$ by scene flow. $\network^\dynamic$ estimates both forwards and backwards scene flow at every point to penalize a bi-direction loss.

%Apart from color and density, the dynamic NeRF also predicts a 3D scene flow value for each point $t$ to the next future time step $f_{i\rightarrow{i+1}}$ and a 3D scene flow value to the previous past time step $f_{i\rightarrow{i-1}}$. 

% Predicted scene flow corresponds each sample point to a corresponding point:
% %
% \begin{equation}
% \label{eq:nsff_scene_flow}
%     % \ray_{i\rightarrow{j}}(\xpos_t) = \ray_i(\xpos_t) + f_{i\rightarrow{j}}(\ray_i(\xpos_t))
%     \ray_{i\rightarrow{j}} = \ray_i + \flow_{i\rightarrow{j}}(\ray_i(\xpos_t))
% \end{equation}

% Thus color output on time step $i$ could be approximated by querying network at time step $j$: $\hat{C}_{j\rightarrow{i}}(r_i)$ according to \ref{color projection}. Assume we starts from $t_n$ as we did in \ref{color integral}, and query all point samples along ray $r_i$ at time step $i$. As we cannot query the network directly for time step $i$, for each point $r_i(t)$ we calculate the corresponding point $r_{i\rightarrow{j}}(t)$ by \ref{scene flow projection}. Then, we use the corresponding point's color prediction $c_j(r_{i\rightarrow{j}}(t)$ and density prediction $\sigma_j(r_{i\rightarrow{j}}(t))$ to replace the color and density in \ref{color integral}, thus we get \ref{color projection}. Note, the transmittance $T_j(t)$ is also calculated using the new density values, but for simplicity we used $T_j(t)$ here.

Thus, we approximate color output at time step $j$ by flowing the queried network values at time step $i$: % $\hat{C}_{j\rightarrow{i}}(r_i)$ according to \ref{color projection}. Assume we starts from $t_n$ as we did in \ref{color integral}, and query all point samples along ray $r_i$ at time step $i$. As we cannot query the network directly for time step $i$, for each point $r_i(t)$ we calculate the corresponding point $r_{i\rightarrow{j}}(t)$ by \ref{scene flow projection}. Then, we use the corresponding point's color prediction $c_j(r_{i\rightarrow{j}}(t)$ and density prediction $\sigma_j(r_{i\rightarrow{j}}(t))$ to replace the color and density in \ref{color integral}, thus we get \ref{color projection}. Note, the transmittance $T_j(t)$ is also calculated using the new density values, but for simplicity we used $T_j(t)$ here.
%
\begin{align}
\label{eq:nsff_loss_color_reprojection}
    % \hat{\xcol}_{j\rightarrow{i}}(r_i) = \int_{t_n}^{t_f} T_j(t)\sigma_j(r_{i\rightarrow{j}}(t))c_j(r_{i\rightarrow{j}}(t), d_i) \, dt
    \pixcol_{i\rightarrow{j}} = \int_{t_n}^{t_f} T_{i\rightarrow j}\sigma_{i\rightarrow j}\xcol_{i\rightarrow j} \, dt
\end{align}

%However, the loss is not always meaningful as 3D scene flow becomes ambiguous when certain 3D location has different occlusion status between two time steps, whereas the temporal photometric consistency loss $L_{pho}$ should not be applied. Taking this phenomena into consideration, the dynamic NeRF predicts two disocclusion weight values $ w_{i\rightarrow{i+1}}$ and $w_{i\rightarrow{i-1}}\in [0, 1]$. Similar to projected color rendering process in \ref{color projection}, the probability of activating $L_{pho}$ is rendered by replacing $c_j(r_{i\rightarrow{j}}(t), d_i)$ with $w_j(r_i(t))$ to get \ref{weight projection}. Note that $w_j(r_i(t))$ is volume rendered along the ray $r_i$ with opacity from time $j$. 

Reprojection must account for occlusion and disocclusion by motion. As such, $\network^\dynamic$ also predicts forwards and backwards scene occlusion weights $w_{i+1}$ and $w_{i-1}\in [0, 1]$, where a point with $w_{i+1}=0$ means that occlusion status is changed one step forwards in time. We can integrate $w$ to a pixel:
%
\begin{align}
\label{eq:nsff_weight_projection}
    % \hat{w}_{i\rightarrow{j}}(r_i) = \int_{t_n}^{t_f} T_j(t)\sigma_j(r_{i\rightarrow{j}}(t))w_j(r_i(t)) \, dt
    \hat{w}_{i\rightarrow{j}} = \int_{t_n}^{t_f} T_{i\rightarrow{j}}\sigma_{i\rightarrow{j}}w_j \, dt 
\end{align}

Then, this pixel weight modulates the color loss such that occluded pixels are ignored. 
\begin{align}
\label{eq:nsff_loss_photometric}
    % \mathcal{L}_{pho} = \sum\limits_{r_i}\sum\limits_{j\in N(i)} \hat{W}_{j\rightarrow{i}}(r_i) &||\hat{C}_{j\rightarrow{i}}(r_i) - C_i(r_i)||_2^2 \nonumber \\
    % + \beta_w \sum\limits_{x_i} &||w_{i\rightarrow{j}}(x_i) - 1||_1
    \lossNSFFPixColProj = \frac{1}{|\mathcal{R}||\mathcal{N}|} \sum\limits_{\ray_i \in \mathcal{R}}\sum\limits_{j\in \mathcal{N}(i)} \hat{w}_{i\rightarrow{j}}(\ray_i) &||\pixcol_{i\rightarrow{j}}(\ray_i) - \pixcol_j^\dagger(\ray_j)||_2^2
\end{align}

To stop the optimization from estimating all-zero occlusion weights, we encourage the weights to be close to one: 
%
\begin{align}
\label{eq:nsff_loss_occlusionweight}
    \lossNSFFw = \frac{1}{|\mathcal{R}|} \sum\limits_{\ray_i \in \mathcal{R}} &||\hat{w}_{i\rightarrow{j}}(\ray_i) - 1||_1
\end{align}

Further, to encourages the 3D scene flow to be cycle consistent, we penalize the difference between forward and backward flowed points across different timesteps. 
% \am{Notation is slightly confusing because $f(x)$ makes me think $f$ is a function rather than a vector.} 
% $f_{i\rightarrow{j}}$ would be consistent with background flow $f_{j\rightarrow{i}}$.
% $L_{cyc}$ is computed ato ensure $f_{i\rightarrow{j}}(x_i) + f_{j\rightarrow{i}}(x_i + f_{i\rightarrow{j}})$ is close to $0$, where $x_i$ are all sampled 3D points. Note that above disocclusion weights $w_{i\rightarrow{j}}$ are used here again as 3D scene flow could be ambiguous due to the disocclusion problem.
%
\begin{align}
\label{eq:nsff_loss_cyclic}
    \lossNSFFCyc = \frac{1}{N} \sum\limits_{\xpos_i}^{N}\sum\limits_{j\in \mathcal{N}(i)} w_{i}||\flowscene_{i}(\xpos_i) + \flowscene_{j}(\xpos_i + \flowscene_{i})||_1
\end{align}


Next, regularizations encourage the scene flow to be small and locally constant.
\begin{align}
\label{eq:nsff_loss_reg}
    \lossNSFFRegFlowSmall &= \frac{1}{N} \sum\limits_{\xpos_i}^{N} ||\flowscene_{i}(\xpos_i)||_1 \\
    % Actually a mean average over n sample points
    \lossNSFFRegFlowSmooth &= \frac{1}{N} \sum\limits_{\xpos_i}^{N} ||\flowscene_{i}(\xpos_i) - \flowscene_{i}(\xpos_i+\epsilon)||_1
\end{align}

Finally, entropy loss encourages the volume rendered blending weights to be completely static or dynamic.
\begin{align}
    \label{eq:nsff_loss_entropy}
    \lossNSFFentropy &= -\frac{1}{|\mathcal{R}|} \sum\limits_{\ray_i \in \mathcal{R}} & {v(\ray_i)\log(v(\ray_i))}
\end{align}

\paragraph{Prior losses}
Reconstructing geometry, appearance, and scene flow given only a monocular video sequence is highly ill posed. Thus, we use the precomputed depth and optical flow maps to penalize reconstruction losses. These decay as optimization progresses to rely more and more on the optimized self-consistent geometry and scene flow. 
% The decay rate on depth and flow losses reduces the influence of any inaccurate pretrained values once the volume is sufficiently formed for the color reprojection and cyclic constraints to be effective, especially on dynamic objects. 

For geometry, we estimate a depth $\hat{d}_i$ for each ray $\ray_i$ by replacing $\xcol_i$ in \cref{eq:nsff_colorintegral} by the distance $t$ along the ray. As the pretrained network produces only relative depth, we estimate a scale and shift for each depth map via transform $z$.
%
\begin{align}
\label{eq:nsff_loss_d}
    \lossNSFFd = \frac{1}{|\mathcal{R}|} \sum\limits_{\ray_i \in \mathcal{R}} ||\hat{d}_i - z(\hat{d}_i^\dagger)||_1
\end{align}

For motion, projecting scene flow to a camera lets us compare to the estimated optical flow. Each sample point along a ray $\xpos_i$ is advected to a point in the neighboring frame $\xpos_{i\rightarrow{j}}$, then integrated to the neighboring camera plane to produce a 2D point offset $\flowoptic_{i}(\ray_i)$. Then, we expect the difference in the start and end positions to match the prior: 
%Weexpected 3D point location $\hat{X}_i(r_i)$, then the corresponding 2D optical flow $\hat{p}_{i\rightarrow{j}}(r_i)$ by perspective projection. Then NSFF force the predicted optical flow $\hat{p}_{i\rightarrow{j}}(r_i)$ to be close to the pseudo groundtruth ${p}_{i\rightarrow{j}}(r_i)$ (\ref{L_{geo}}).
%
\begin{align}
\label{eq:nsff_loss_opticalflow}
    \lossNSFFof = \frac{1}{|\mathcal{R}||\mathcal{N}|} \sum\limits_{\ray_i \in \mathcal{R}}\sum\limits_{j\in \mathcal{N}(i)} ||\flowoptic_{i}(\ray_i) - \flowoptic^\dagger_{i}(\ray_i)||_1
\end{align}

The final combined objective is then:
%
\begin{align}
\label{eq:nsff_finalloss}
    \lossNSFF = \lossNSFFPixCol 
    + \lambdaNSFFPixColProj \lossNSFFPixColProj
    + \lambdaNSFFw      \lossNSFFw 
    + \lambdaNSFFCyc    \lossNSFFCyc \nonumber \\
    + \lambdaNSFFRegFlowSmall    \lossNSFFRegFlowSmall
    + \lambdaNSFFRegFlowSmooth   \lossNSFFRegFlowSmooth
    + \lambdaNSFFd      \lossNSFFd
    + \lambdaNSFFof     \lossNSFFof
    + \lambdaNSFFentropy \lossNSFFentropy
\end{align}


==> tex/03e_methods_implementation.tex <==
\section{Implementation Details}
\label{sec:implementation}

\paragraph{Semantics and Attention}

Following Amir \etal~\cite{amir2021deep}, for semantics we extract the 384-dim.~`key' facet from the \nth{11} layer of \semfeatnetwork, and for saliency we extract the 1-dim.~`attention' facet from the \nth{11} layer.
%
For the pyramid, we use three levels. The coarsest level 0 is downsampled to $240\times 128$. The finest level 2 is the input RGB size, with the mid level 1's size set between the two. For each level, we use \semfeatnetwork as a sliding window of size $240\times 128$ to extract a (8$\times$8 patch; stride 4) $60\times 32$ feature map (i.e., level 0 has only one window position). For fast computation, we set window stride to 64. Once extracted, we upsample and place each feature map within level 2's frame. Then, for each pixel, we mean average all features from all windows that intersected it.
% 's window size is $480\times 256$, while top level's window size is $240\times 128$. For each level, we select the stride to be half of the window size. For each window, we interpolate the content to be $240\times 128$, extract \semfeatnetwork features, interpolate the feature back to original window size, then mean average the features across windows that intersect each pixel. 
%
Finally, to fit within GPU VRAM, we perform PCA on all images' normalized extracted pyramid $\hat{\semfeat},\hat{\attfeat}$ features and keep the most important 64 dimensions. 
% Empirically, this does not hurt performance because each video's content only comes from some limited semantic space.

\paragraph{Clustering}
Any clustering method has hyperparameters (or thresholds) for it to make decisions about cluster assignment. We use the same hyperparameters for all sequences.


We use the GPU via Faiss~\cite{johnson2019billion}. Again to fit within GPU VRAM, we uniformly sample every fifth point for elbow-$k$ finding, then propagate cluster assignment to all points given $k$. We set the elbow-$k$ threshold to 0.975 and the max cluster number to 25, with 10 trials per $k$. We cluster on direction and so normalize each pixel's vector.

\paragraph{Object extraction}
To extract an object from the volume, we sample 3D points along each input ray, then compare their semantics to to existing projected 2D semantic cluster centroids. We assign each 3D point to its closest centroid. Then, we set non-salient cluster label points to have zero density.

% For each input image ray's volume point sample ($W\!\!\times\!\!H\times\!\!\#samples$), we query all fields, then assign each 3D point a cluster label given its feature and fitted centroids 
% \jt{semantic feature? do we do this by matching to the cluster centroids via cosine similarity?}. 
% We simply set non-salient cluster label points to have zero volume density. Then, we can render the extracted object at novel space-time views.
% % Post-processing: given rendered blending map, set map with value $<0.1$ locations to be black in color image
% On the rendered 2D color/depth image, we set all pixels that are assigned background label to be black/0.

\paragraph{Post process}
All quantitative results are \emph{without} this unless stated; only the main paper Table 3 line includes this. 
%As we want salient objects, we morphologically open and close (3$\times$3) projected clusters and then merge remaining small clusters ($<\!\!\!0.01\times\!$ image area) into their nearest neighbors.
As appearance and geometry information is embedded in the volume, we want to refine the decomposition results by constraining them to align with rendered RGB and depth images. Specifically, we apply a CRF~\cite{NIPS2011_beda24c1} with a pairwise Gaussian unary potential ($\theta_{\gamma}$=$3$, $w$=$15$), a pairwise bilateral RGB potential ($\theta_{\gamma}$=$40$, $\theta_{\beta}$=$13$, $w$=$10$), and a pairwise bilateral depth potential ($\theta_{\gamma}$=$40$, $\theta_{\beta}$=$13$, $w$=$20$).
Applying a CRF is similar to Amir et al.~\cite{amir2021deep} on \semfeatnetwork in 2D, but our spacetime volume-integrated geometry provides a much stronger constraint on where the true edge is over time.
% We do not refine edges beyond this (cf.~\cite{amir2021deep}). 
The contribution of post processing is showed in \cref{fig:postprocessed} qualitatively. We see that small unimportant regions are removed, while still maintaining thin features and fine details. This trade-off is an application-level decision.
% , merge semantic clusters with more than $x$ unconnected islands, and 
% 540 x 288 

\input{fig/fig_post/fig_post.tex}

% During object extraction, we also obtain the corresponding segmentation mask without setting the density to be zero. This tells us whether each pixel will be background in a particular view. After extracting the object and rendering 2D color images, we set the background pixels to be transparent.  

\paragraph{Optimization routine and hyperparameters}

We optimize the combined loss with Adam optimizer, learning rate $5e^{-4}$, $\beta=(0.9$, $0.999)$. We multiply prior losses for depth and optical flow by a decay rate. This rate starts at 1 and is divided by 10 at every 300,000$^{\text{th}}$ iteration.
%
% Code for decay scheme; optimization iteration i
% decay_iteration = 30
% divsor = i // (decay_iteration * 1000)
% decay_rate = 10
% if args.decay_depth_w:
%     w_depth = args.w_depth/(decay_rate ** divsor)
% else:
%     w_depth = args.w_depth
%
For \titlename, we set reprojection losses $\lambdaSAFFsemproj=1.0$ and $\lambdaSAFFattproj=1.0$, and prior losses $\lambdaSAFFsem=0.04$ and $\lambdaSAFFatt=0.04$~\cite{kobayashi2022distilledfeaturefields}. For all other losses, we follow Li et al.~\cite{li2020neural}:  %
$\lambdaNSFFRegFlowSmall = 0.1$,
$\lambdaNSFFRegFlowSmooth = 0.1$,
$\lambdaNSFFw = 0.1$,
$\lambdaNSFFPixColProj = 1.0$,
$\lambdaNSFFCyc = 1.0$,
$\lambdaNSFFd = 0.04$,
$\lambdaNSFFof = 0.02$,
$\lambdaNSFFentropy = 0.001$.

\titlename, its ablations, and NSFF are optimized for $360$k iterations. As \ddnerf is a different architecture, we use the author's stated $100$k iterations.

\paragraph{Computational cost.}
The code was developed on Ubuntu 20.10 in Python/PyTorch, and trained on NVIDIA GeForce RTX 3090, NVIDIA GeForce RTX A6000, and NVIDIA GeForce RTX 2080 TI GPUs. All operations assume access to only $1$ GPU. The CUDA VRAM required for using a trained \titlename on $540\times 288$ image size is $12$ GB, while optimization requires $24$ GB. 
% The minimum cuda memory required for using \titlename drops to $12$ GB when image size shrinks to $128*128$. 
The CPU RAM used to optimize, cluster, and render \titlename used $16$ GB, while we use $36$ GB to extract objects. 
Optimizing a \titlename for $360,000$ iterations takes $1$ to $2$ days, depending on hardware, and is similar in time to NSFF. Recent improvements have dramatically reduced this time for non-semantic-attention fields~\cite{muller2022instant,chen2022tensorf}, and we expect similar performance gains were these methods used as the underlying architecture. In terms of runtime, we preprocess the \semfeatnetwork features and so do not incur significant additional cost during optimization, and none during inference due to \semfeatnetwork. Per-frame rendering is 15\% slower than NSFF due to the additional heads. Saliency-aware clustering takes a few seconds only.

The computational cost is currently expensive, but we see our work as a step towards integrating high and low level information for 4D semantic volume reconstruction. NeRF-based approaches are still some way from real-time performance, but there have been significant gains recently (e.g., InstantNGP~\cite{muller2022instant}). Building our approach upon a fast backbone like this would make our approach more practical. One additional note is that, versus supervised 2D segmentation networks that are typically trained to be feed forward and to make predictions quickly (e.g., ProposeReduce takes only a few seconds to process a short sequence), the output of our model is richer as a 4D reconstruction with time-varying correspondence.

With respect to scalability, longer sequences will take more time to process, and at some point the capacity of the MLPs will limit reconstruction detail. For scenes with more dynamic elements, many objects are not in principle a problem, but instances that spatially overlap cannot be separately determined due to the fact that DINO-ViT features are not instance-aware.

\paragraph{Network architecture}
We add two heads to the architecture of NSFF~\cite{li2020neural}. For the semantic head, we add a single linear layer (256 neurons) appended by a tanh layer, with output dimension 64 to match the size of the per-sequence PCA-reduced \semfeatnetwork features. For the saliency head, we add a single linear layer (256 neurons) appended by a sigmoid layer, with output dimension 1. 

%\vspace{-0.15cm}
%\paragraph{Pseudocodes}
%We include the saliency-aware clustering (Alg.~\ref{alg:cluster}) and the pyramid construction (Alg.~\ref{alg:pyr_final}).

==> tex/03f_methods_designchoices.tex <==
\section{Design Choices}
\label{sec:designchoices}

\subsection{Underlying Dynamic NeRF Approach}

\paragraph{View synthesis and depth}
First, we evaluate whether RGB view synthesis performance is affected by adding more heads to the MLP. We find that it is not affected (\cref{tab:rgb_noharm}). \ddnerf's hyper-spacetime deformation has trouble reconstructing images on this dataset, producing distorted dynamic objects or failing to freeze time. 
% For scene geometry over time (depth), we produce similar results to NSFF (cf.~in our supplement).

In \cref{fig:viewsynthesis_rgbdepth}, we show qualitatively that \titlename does not degrade view synthesis or depth quality compared to NSFF~\cite{li2020neural}, while \ddnerf struggles with our data.

\paragraph{Why does \ddnerf struggle?} 
The main distinction is that \ddnerf is a deformation-based method while NSFF and \titlename are flow-based methods. For \ddnerf, the scene is reconstructed in a canonical space and deformed to render the results. \ddnerf struggles with larger motion in the scene---in the NVIDIA dataset, it is notably more difficult to find temporal correspondence within because frames are spatially far apart (unlike other monocular datasets created from one video camera only). Given only a monocular video to describe a scene with large camera motion \emph{and} large object motion, it appears difficult to faithfully reconstruct both the canonical space and the deformation. 
In comparison, \ddnerf produces good RGB reconstructions on the Nerfies~\cite{park2021nerfies} dataset because both the camera and scene motion are smaller than in the NVIDIA Dynamic Scene Dataset.

% View synthesis experiment
\input{tab/tab_rgb_noharm.tex}

\input{fig/fig_rgb/fig_rgb.tex}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\clearpage % new page
\subsection{3D vs.~2D Projected vs.~4D Spacetime Clustering}
\label{sec:spacetime4Dclustering}

In our saliency-aware clustering step, the elbow $k$-means method can take as input the per-pixel semantics features that have been sampled from 3D points in the volume (\textbf{in 3D}), or that have been rendered from the volume back to the 2D plane. Even though a volume is reconstructed, we find performance is somewhat worse when clustering in 3D than in projected 2D space (\cref{tab:spacetime4dclustering}; and in main paper). With respect to evaluation, it is difficult to collect ground truth segmented 3D data for dynamic real world scenes (none exist to our knowledge); this remains future work.

So, why might clustering in 3D lead to worse segmentations? Given monocular input from narrow baselines and dynamic scenes, the reconstruction can be imprecise with noisy geometry. This is in contrast to dynamic scenes captured with multi-camera setups or static scenes captured with wide baselines. 
% Thus, precise separation in 3D from monocular casually-captured videos is hard, leading to better clustering performance in volume-projected spacetime. 
%In the monocular input case with narrow baselines and dynamic scenes, it is challenging to precisely reconstruct geometries. 
As semantics and saliency use the same estimated geometry as radiance, clustering in the 3D volume introduces inaccuracy in the decomposition result, thus reducing the performance quantitatively and qualitatively. We visualize the volume as a point cloud from sampled 3D points in ~\cref{fig:fig3Dnoise}. Although the volume looks natural from the training view, erroneous regions are visible when the camera pose is far away from the training view, especially on the dynamic objects. 
%The incorrect geometry at those regions introduces noise into both semantics and saliency fields. }

Given direct clustering in 3D suffers from the narrow-baseline issue, we introduce another variant (\textbf{in 4D spacetime}) that also clusters upon a 3D position for each input pixel using the recovered volume density (from the estimated depth) and the timestep. While not the same as a volumetric clustering with some dense sampling, this sparse alternative is a reasonable computational compromise as our scenes contain opaque objects without participating media. We concatenate the spacetime coordinates with the semantic features for each pixel, then empirically adjust their relative weights to increase foreground segmentation performance.

In principle, this could exploit the underlying geometry to provide better edges or more instance awareness to the method. However, in practice, this does not reliably happen (\cref{tab:spacetime4dclustering}). 
Any error in alignment between the semantic information and the geometry causes the clustering to confuse elements, e.g., semantics for the same object at different depths over edge boundaries. As a consequence, semantically-different entities may not be correctly separated (\seqTruck), or are missing parts (\seqJumping, \cref{fig:spacetime4dclustering}). As such, we use only projected 2D semantic features as input to the clustering.

However, even though we use semantic-attention pyramids to increase the geometric resolution of the \semfeatnetwork features significantly, and even though volume integration increases these still (e.g., main paper, Figure 2), one might ask whether the optimization routine could also help further align the geometry and semantic features during volume integration. This brings us to the next subsection.

\input{tab/tab_spacetime4Dclustering.tex}
\input{fig/fig_3D_noise/fig_3D_noise}
\input{fig/fig_spacetime4Dclustering/fig_spacetime4Dclustering.tex}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\clearpage % new page
\subsection{Decaying Semantics and Attention}
\label{sec:decaysemantics}

One way to improve the alignment of depth edges and semantic and attention features is through decaying their reconstruction loss through training. This decay happens to the depth and optical flow priors, and for those channels of information the decay provides freedom to the optimization to refine the spacetime density once initialized with respect to the self-consistent multi-view and scene flow constraints. Intuitively, decaying the semantics and attention reconstructions would also provide more freedom to further optimize the spacetime density to minimize the self-consistent multi-view and scene flow constraints when the semantics disagreed. 

However, in the main paper, we describe that semantics and attention are not priors---there is no self-consistency for semantics to constrain their values, thus, after decay the optimization is free for them to vary inconsistently and so for their reprojection to lose useful meaning. This could have unwanted consequences.

To investigate this design choice, we implement variant \textbf{w/ decay} in which we use the same decaying mechanism as depth and optical flow on $\lossSAFFsem$ and $\lossSAFFatt$. 
We also decay $\lossSAFFsemproj$ and $\lossSAFFattproj$, because the semantics are not necessarily consistent with the spacetime geometry.
% \jt{Find argument for why we also decay scene flow losses.}

% \jt{Yiqing, why do we decay the semantic flow loss? We want to keep that. We only want to decay the reconstruction loss. NSFF doesn't decay the flow losses.}
% \YL{argument(one sure side-effect): decayed semantics and attention fields are not exactly "correct"; in this case not decaying their flow may erroneously twist them to do their best to match the flow constrains but degrade to meaningless values }

Qualitatively, adding decay does better align the semantics and attention fields with the geometry, e.g., in \seqSkating, the space between skater's legs are better segmented; however, the clustering performance degrades all over the image (\cref{fig:decay}), e.g., in \seqSkating, now including a sconce and unwanted floor details (zoom in). This is also reflected quantitatively (\cref{tab:decay}).

\input{fig/fig_decay/fig_decay.tex}
\input{tab/tab_decay.tex}

\vfill


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\clearpage % new page
\subsection{Pyramid Construction}
\label{sec:pyramidconstruction}


Figure~\ref{fig:pyramidconstruction} provides a diagrammatic example for how we construct our feature pyramids. We also provide algorithm pseudocode (\cref{alg:pyr_final}).

As mentioned in the main paper, given the pyramid layers, we begin conceptually from a weighted sum of three layers for semantics using $\lambdaSAFFsem\! =\! \{\nicefrac{1}{3},\nicefrac{1}{3},\nicefrac{1}{3} \}$ and with coarsest whole-image attention with $\lambdaSAFFatt\! =\! \{1,0,0\}$. This already gives quantitatively better decomposition performance than without using a pyramid (\textbf{w/o pyr}; \cref{tab:pyramiddecompose}). However, the optimized semantic field does not correspond as well to scene geometry and is more influenced by error in the coarsest layer semantics and attention than our approach. For instance, the human is not identified as salient in \seqBalloonNoticeBoard (\cref{fig:pyramid_compare}). Additionally, as the finer layer sliding windows do not typically contain the object of interest in boundary regions, the extracted features are incorrect. This causes unwanted clusters to appear around image edges, e.g., the gray cluster in the top right corner in \seqUmbrella (\cref{fig:pyramid_compare}).

To increase semantic and attention resolution, we increase $\lambdaSAFFsem\!$'s dependency on finer layers to $\! \{\nicefrac{4}{9},\nicefrac{4}{9},\nicefrac{1}{9} \}$. To deal with the boundary issues, we decrease the weight of fine layers towards the boundary back to $\! \{\nicefrac{1}{3},\nicefrac{1}{3},\nicefrac{1}{3} \}$. The image boundary problem is resolved in \seqUmbrella (\cref{fig:pyramid_compare}). However, there is still a mismatch between the fidelity of the semantics and saliency (the head disappears in \seqDynamicFace), which is also reflected quantitatively (\cref{tab:pyramiddecompose}).

Thus, we use the same weight proportions and boundary reduction for both semantics and attention. This strikes a balance between correct edges from fine layers and whole object features from coarse layers, and mitigates the feature noise around image boundaries. This yields the best overall results both qualitatively on balance (\cref{fig:pyramid_compare}) and quantitatively (\cref{tab:pyramiddecompose}).

% Force a new column so that the table is on the right.
\newpage

\input{fig/fig_pyramiddiagram/fig_pyramiddiagram}
\input{tab/tab_pyramid.tex}

\input{fig/fig_pyramid/fig_pyramid.tex}
\input{alg/alg_pyramid_new}

%Practically, we use \cref{alg:pyr_final} to compute the pyramid.

%\jt{Write condition names in Figure in this paragraph.}


==> tex/styleguide.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Style guide
%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Terminology / understanding
%
% 1. Saliency is a concept 
% 2. Attention are features
%
% 3. The process of using the volume is called `volume integration'.
%    It is not called `distillation' because we are not trying to 
%    find a reduced dimensionality form of the features that 
%    represent as much information as the input dimensionality.
%
% 4. We do not `train' a SAFF, there is no `learning'.
%    We optimize a SAFF.
%
% 5. For data, there is no `training set' or `test set'.
%    There are input views and hold-out views.
%
%
%
% n. We do not `prove' anything; this is not theory.
%    We `provide evidence for' or `demonstrate'. 
%    `Show' is on the edge ; )
%    Always use measured language.
%
% n. No weasel words. Do not use `very' or `clearly'.
%    State it plainly without presumption.

==> tex/tex_necv.tex <==

%\YL{Set the context; ground the scenario}
Given a casually-captured monocular RGB video, decomposing its depicted real-world dynamic scene into foreground objects and background is an important task in computer vision, with downstream applications in segmentation and beyond such as in video editing. Ideally, we would also reconstruct the geometry and appearance over time, including its frame-to-frame correspondence.

%\YL{Talk about other works' limitation}
Previous methods have made great progress in these directions but there are many challenges. Some works assumes that there is no object motion in the scene, or take input from multi-view cameras, or do not explicitly reconstruct the underlying 3D structure of the scene. For objects, some works rely on masks or user input to aid segmentation, or use task-specific training datasets. 
Sometimes, works assume a number of object slots ahead of time. Given the challenges, many works train and test on synthetic data.

%\YL{Talk about our method and why can solve}
To overcome the challenges, we integrate low-level reconstruction cues with high-level pretrained information---bottom-up and top-down---into neural volumes. Specifically, we consider the added value of embedded semantic and saliency (attention) information for dynamic scene decomposition. Our semantic attention flow fields (\titlename) build upon the neural scene flow fields approach~\cite{li2020neural}. For optimization, we supervise two network heads with pretrained \semfeatnetwork~\cite{caron2021emerging} semantic features and attention. To extract higher-fidelity information from low-resolution \semfeatnetwork output, we build a semantic attention pyramid that trades detail with whole-image context. Having optimized a \titlename representation for a dynamic scene, we perform a saliency-aware clustering on rendered feature images to describe objects and their background. Given the volume reconstruction, the clustering generalizes to novel spacetime views.

%\YL{List our findings}
To evaluate \titlename's dynamic scene decomposition capacity, we expand the NVIDIA Dynamic Scene Dataset \cite{Yoon_2020_CVPR} by manually annotating object masks across input and hold-out views. We demonstrate that \titlename outperforms 2D \semfeatnetwork baselines and is comparable to  a state-of-the-art video segmentation method ProposeReduce\cite{lin2021video} on our data. 

\vspace{-0.2cm}



